Vanadium Abundance Derivations in 255 Metal-poor Stars

We present vanadium (V) abundances for 255 metal-poor stars, derived from high-resolution optical spectra from the Magellan Inamori Kyocera Echelle spectrograph on the Magellan Telescopes at Las Campanas Observatory, the Robert G. Tull Coud\'{e} Spectrograph on the Harlan J. Smith Telescope at McDonald Observatory, and the High Resolution Spectrograph on the Hobby-Eberly Telescope at McDonald Observatory. We use updated V I and V II atomic transition data from recent laboratory studies, and we increase the number of lines examined (from 1 to 4 lines of V I, and from 2 to 7 lines of V II). As a result, we reduce the V abundance uncertainties for most stars by more than 20% and expand the number of stars with V detections from 204 to 255. In the metallicity range $-$4.0 $<$ [Fe/H] $< -$1.0, we calculate the mean ratios [V I/Fe I]$ = -0.10 \pm 0.01 (\sigma = 0.16)$ from 128 stars with $\geq$ 2 V I lines detected, [V II/Fe II] $= +0.13 \pm 0.01 (\sigma = 0.16)$ from 220 stars with $\geq$ 2 V II lines detected, and [V II/V I] $= +0.25 \pm 0.01 (\sigma = 0.15)$ from 119 stars. We suspect this offset is due to non-LTE effects, and we recommend using [V II/Fe II], which is enhanced relative to the solar ratio, as a better representation of [V/Fe]. We provide more extensive evidence for abundance correlations detected previously among scandium, titanium, and vanadium, and we identify no systematic effects in the analysis that can explain these correlations.

==> tab02.tex <==
% Too long; maybe don't include the whole table
\startlongtable
\begin{deluxetable}{cccc}
\tablecaption{Abundances Derived from Neutral Vanadium Lines
\label{v1tab}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Star} &
\colhead{Wavelength (\AA)} &
\colhead{\log \epsilon (V~\textsc{i})} &
\colhead{$\sigma$}
}
\startdata
      BD~$+$10\degree2495 &        4111.779 &            1.51 &            0.10 \\ 
      BD~$+$10\degree2495 &        4379.230 &            1.39 &            0.06 \\ 
      BD~$+$10\degree2495 &        4389.979 &            1.42 &            0.10 \\ 
      BD~$+$10\degree2495 &        4408.196 &            1.33 &            0.20 \\ 
     BD~$+$19\degree1185a &        4111.779 &            2.44 &            0.20 \\ 
     BD~$+$19\degree1185a &        4379.230 &            2.53 &            0.10 \\ 
     BD~$+$19\degree1185a &        4389.979 &            2.56 &            0.15 \\ 
     BD~$+$19\degree1185a &        4408.196 &            2.38 &            0.10 \\ 
      BD~$+$26\degree3578 &        4379.230 &            1.43 &            0.10 \\ 
      BD~$+$29\degree2356 &        4111.779 &            1.96 &            0.10 \\ 
      BD~$+$80\degree0245 &        4379.230 &            1.28 &            0.10 \\ 
      BD~$-$01\degree2582 &        4111.779 &            1.01 &            0.10 \\ 
     BD~$-$15\degree5781 &        4111.779 &            0.69 &            0.10 \\ 
     BD~$-$15\degree5781 &        4379.230 &            0.66 &            0.10 \\ 
     BD~$-$15\degree5781 &        4389.979 &            0.87 &            0.06 \\ 
     BD~$-$15\degree5781 &        4408.196 &            0.69 &            0.15 \\ 
      BD~$-$18\degree5550 &        4379.230 &            0.65 &            0.06 \\ 
     BD~$-$20\degree6008 &        4111.779 &            0.76 &            0.10 \\ 
     BD~$-$20\degree6008 &        4379.230 &            0.52 &            0.20 \\ 
     BD~$-$20\degree6008 &        4389.979 &            0.64 &            0.10 \\ 
     BD~$-$20\degree6008 &        4408.196 &            0.52 &            0.15 \\ 
     CD~$-$24\degree1782 &        4111.779 &            0.85 &            0.15 \\ 
     CD~$-$24\degree1782 &        4379.230 &            0.70 &            0.15 \\ 
     CD~$-$24\degree1782 &        4389.979 &            0.97 &            0.30 \\ 
     CD~$-$36\degree1052 &        4111.779 &            2.25 &            0.15 \\ 
     CD~$-$36\degree1052 &        4379.230 &            2.07 &            0.15 \\ 
     CD~$-$36\degree1052 &        4389.979 &            1.95 &            0.15 \\ 
     CD~$-$36\degree1052 &        4408.196 &            2.16 &            0.30 \\ 
      CS~22166-016 &        4111.779 &            0.80 &            0.20 \\ 
      CS~22166-016 &        4379.230 &            0.65 &            0.15 \\ 
      CS~22166-016 &        4389.979 &            0.50 &            0.20 \\ 
      CS~22169-008 &        4389.979 &            1.46 &            0.10 \\ 
      CS~22169-035 &        4111.779 &           -0.16 &            0.20 \\ 
      CS~22169-035 &        4379.230 &            0.08 &            0.10 \\ 
      CS~22169-035 &        4389.979 &            0.29 &            0.30 \\ 
      CS~22169-035 &        4408.196 &            0.29 &            0.30 \\ 
      CS~22171-031 &        4379.230 &            1.51 &            0.30 \\ 
      CS~22172-029 &        4111.779 &            1.14 &            0.05 \\ 
      CS~22172-029 &        4379.230 &            1.08 &            0.06 \\ 
      CS~22172-029 &        4389.979 &            1.05 &            0.10 \\ 
      CS~22172-029 &        4408.196 &            0.90 &            0.50 \\ 
      CS~22180-014 &        4111.779 &            1.31 &            0.40 \\ 
      CS~22180-014 &        4379.230 &            1.38 &            0.20 \\ 
      CS~22182-033 &        4379.230 &            1.41 &            0.10 \\ 
      CS~22182-047 &        4111.779 &            1.79 &            0.10 \\ 
      CS~22182-047 &        4379.230 &            1.79 &            0.06 \\ 
      CS~22183-031 &        4111.779 &            0.43 &            0.10 \\ 
      CS~22183-031 &        4379.230 &            0.49 &            0.06 \\ 
      CS~22183-031 &        4389.979 &            0.73 &            0.30 \\ 
      CS~22185-007 &        4111.779 &            0.89 &            0.10 \\ 
      CS~22185-007 &        4379.230 &            0.83 &            0.06 \\ 
      CS~22185-007 &        4389.979 &            0.74 &            0.15 \\ 
      CS~22186-002 &        4379.230 &            1.20 &            0.10 \\ 
      CS~22186-017 &        4379.230 &            1.39 &            0.10 \\ 
      CS~22186-017 &        4389.979 &            1.81 &            0.20 \\ 
      CS~22186-023 &        4111.779 &            0.71 &            0.10 \\ 
      CS~22186-023 &        4379.230 &            0.62 &            0.06 \\ 
      CS~22189-009 &        4111.779 &           -0.11 &            0.30 \\ 
      CS~22189-009 &        4379.230 &           -0.20 &            0.10 \\ 
      CS~22873-128 &        4111.779 &            0.63 &            0.10 \\ 
      CS~22873-128 &        4379.230 &            0.60 &            0.10 \\ 
      CS~22873-128 &        4389.979 &            0.60 &            0.10 \\ 
      CS~22876-040 &        4379.230 &            2.03 &            0.10 \\ 
      CS~22877-001 &        4379.230 &            0.20 &            0.06 \\ 
      CS~22877-011 &        4111.779 &            0.78 &            0.10 \\ 
      CS~22877-011 &        4379.230 &            0.71 &            0.06 \\ 
      CS~22877-011 &        4389.979 &            0.65 &            0.30 \\ 
      CS~22877-015 &        4379.230 &            1.78 &            0.30 \\ 
      CS~22878-101 &        4379.230 &            0.36 &            0.06 \\ 
      CS~22879-029 &        4379.230 &            1.60 &            0.20 \\ 
      CS~22879-097 &        4379.230 &            1.82 &            0.30 \\ 
      CS~22879-103 &        4111.779 &            1.51 &            0.10 \\ 
      CS~22879-103 &        4379.230 &            1.81 &            0.10 \\ 
      CS~22879-103 &        4389.979 &            1.51 &            0.20 \\ 
      CS~22879-103 &        4408.196 &            1.96 &            0.30 \\ 
      CS~22880-086 &        4379.230 &            0.59 &            0.30 \\ 
      CS~22880-086 &        4389.979 &            0.59 &            0.40 \\ 
      CS~22881-036 &        4379.230 &            1.77 &            0.20 \\ 
      CS~22882-001 &        4389.979 &            1.97 &            0.25 \\ 
      CS~22882-006 &        4379.230 &            1.37 &            0.20 \\ 
      CS~22883-037 &        4111.779 &            1.89 &            0.10 \\ 
      CS~22883-037 &        4379.230 &            1.89 &            0.20 \\ 
      CS~22883-037 &        4389.979 &            1.68 &            0.20 \\ 
      CS~22884-020 &        4111.779 &            1.66 &            0.20 \\ 
      CS~22884-020 &        4379.230 &            1.66 &            0.06 \\ 
      CS~22886-012 &        4379.230 &            1.48 &            0.20 \\ 
      CS~22886-044 &        4111.779 &            1.85 &            0.20 \\ 
      CS~22886-044 &        4379.230 &            2.30 &            0.06 \\ 
      CS~22886-044 &        4408.196 &            1.85 &            0.05 \\ 
      CS~22888-047 &        4379.230 &            1.15 &            0.20 \\ 
      CS~22890-011 &        4379.230 &            1.40 &            0.20 \\ 
      CS~22890-024 &        4111.779 &            1.06 &            0.10 \\ 
      CS~22890-024 &        4379.230 &            1.06 &            0.30 \\ 
      CS~22890-024 &        4389.979 &            1.21 &            0.20 \\ 
      CS~22891-184 &        4379.230 &            1.11 &            0.30 \\ 
      CS~22891-209 &        4111.779 &            0.36 &            0.30 \\ 
      CS~22891-209 &        4379.230 &            0.36 &            0.20 \\ 
      CS~22891-209 &        4389.979 &            0.48 &            0.10 \\ 
      CS~22891-221 &        4379.230 &            0.63 &            0.30 \\ 
      CS~22892-052 &        4111.779 &            0.32 &            0.10 \\ 
      CS~22892-052 &        4379.230 &            0.32 &            0.10 \\ 
      CS~22893-005 &        4111.779 &            1.24 &            0.20 \\ 
      CS~22893-005 &        4379.230 &            1.00 &            0.20 \\ 
      CS~22893-011 &        4379.230 &            1.81 &            0.10 \\ 
      CS~22896-015 &        4111.779 &            1.09 &            0.20 \\ 
      CS~22896-015 &        4379.230 &            1.06 &            0.20 \\ 
      CS~22896-015 &        4389.979 &            0.91 &            0.20 \\ 
      CS~22896-110 &        4111.779 &            1.30 &            0.30 \\ 
      CS~22896-110 &        4379.230 &            1.24 &            0.10 \\ 
      CS~22897-008 &        4111.779 &            0.37 &            0.40 \\ 
      CS~22897-008 &        4379.230 &            0.07 &            0.30 \\ 
      CS~22897-008 &        4389.979 &            0.40 &            0.30 \\ 
      CS~22898-047 &        4379.230 &            0.47 &            0.20 \\ 
      CS~22937-072 &        4111.779 &            1.52 &            0.10 \\ 
      CS~22937-072 &        4379.230 &            1.22 &            0.10 \\ 
      CS~22937-072 &        4389.979 &            1.58 &            0.10 \\ 
      CS~22940-070 &        4111.779 &            2.22 &            0.20 \\ 
      CS~22940-070 &        4379.230 &            2.46 &            0.06 \\ 
      CS~22940-070 &        4389.979 &            2.52 &            0.20 \\ 
      CS~22940-070 &        4408.196 &            2.67 &            0.30 \\ 
      CS~22940-077 &        4379.230 &            1.32 &            0.15 \\ 
      CS~22940-121 &        4379.230 &            1.12 &            0.10 \\ 
      CS~22941-017 &        4111.779 &            0.82 &            0.20 \\ 
      CS~22941-017 &        4379.230 &            1.03 &            0.30 \\ 
      CS~22942-002 &        4379.230 &            0.16 &            0.30 \\ 
      CS~22942-011 &        4111.779 &            0.67 &            0.20 \\ 
      CS~22942-011 &        4379.230 &            0.70 &            0.20 \\ 
      CS~22942-011 &        4389.979 &            0.82 &            0.30 \\ 
      CS~22942-035 &        4111.779 &            0.88 &            0.20 \\ 
      CS~22942-035 &        4379.230 &            0.73 &            0.06 \\ 
      CS~22942-035 &        4389.979 &            0.58 &            0.20 \\ 
      CS~22943-095 &        4379.230 &            1.50 &            0.10 \\ 
      CS~22943-132 &        4111.779 &            1.56 &            0.30 \\ 
      CS~22943-132 &        4379.230 &            1.41 &            0.30 \\ 
      CS~22944-032 &        4111.779 &            0.84 &            0.05 \\ 
      CS~22944-032 &        4379.230 &            0.78 &            0.06 \\ 
      CS~22944-032 &        4389.979 &            0.54 &            0.20 \\ 
      CS~22945-024 &        4379.230 &            1.34 &            0.10 \\ 
      CS~22945-028 &        4111.779 &            0.94 &            0.15 \\ 
      CS~22945-028 &        4379.230 &            0.73 &            0.20 \\ 
      CS~22945-028 &        4389.979 &            1.00 &            0.10 \\ 
      CS~22945-063 &        4379.230 &            1.19 &            0.10 \\ 
      CS~22947-187 &        4111.779 &            1.32 &            0.15 \\ 
      CS~22947-187 &        4379.230 &            1.17 &            0.20 \\ 
      CS~22947-187 &        4389.979 &            1.32 &            0.10 \\ 
      CS~22948-066 &        4379.230 &            0.66 &            0.20 \\ 
      CS~22948-066 &        4389.979 &            0.99 &            0.30 \\ 
      CS~22949-037 &        4379.230 &           -0.02 &            0.30 \\ 
      CS~22949-037 &        4389.979 &            0.01 &            0.20 \\ 
      CS~22949-048 &        4111.779 &            0.43 &            0.20 \\ 
      CS~22949-048 &        4379.230 &            0.22 &            0.10 \\ 
      CS~22949-048 &        4389.979 &            0.19 &            0.20 \\ 
      CS~22950-046 &        4379.230 &           -0.31 &            0.20 \\ 
      CS~22951-059 &        4379.230 &            0.78 &            0.30 \\ 
      CS~22951-059 &        4389.979 &            0.99 &            0.10 \\ 
      CS~22951-077 &        4111.779 &            1.25 &            0.05 \\ 
      CS~22951-077 &        4379.230 &            1.37 &            0.06 \\ 
      CS~22951-077 &        4389.979 &            1.22 &            0.10 \\ 
      CS~22951-077 &        4408.196 &            1.40 &            0.20 \\ 
      CS~22952-015 &        4379.230 &           -0.02 &            0.20 \\ 
      CS~22953-003 &        4111.779 &            0.69 &            0.15 \\ 
      CS~22953-003 &        4379.230 &            0.39 &            0.20 \\ 
      CS~22953-003 &        4389.979 &            0.51 &            0.10 \\ 
      CS~22954-015 &        4379.230 &            1.92 &            0.20 \\ 
      CS~22955-110 &        4379.230 &            2.77 &            0.06 \\ 
      CS~22955-110 &        4389.979 &            2.58 &            0.10 \\ 
      CS~22955-110 &        4408.196 &            2.62 &            0.20 \\ 
      CS~22956-050 &        4379.230 &           -0.02 &            0.20 \\ 
      CS~22956-050 &        4389.979 &            0.28 &            0.30 \\ 
      CS~22956-062 &        4111.779 &            1.24 &            0.20 \\ 
      CS~22956-062 &        4379.230 &            1.04 &            0.10 \\ 
      CS~22956-114 &        4111.779 &            0.55 &            0.30 \\ 
      CS~22956-114 &        4379.230 &            0.64 &            0.10 \\ 
      CS~22957-013 &        4111.779 &            0.72 &            0.10 \\ 
      CS~22957-013 &        4379.230 &            0.51 &            0.10 \\ 
      CS~22957-019 &        4379.230 &            1.62 &            0.20 \\ 
      CS~22957-022 &        4111.779 &            0.76 &            0.40 \\ 
      CS~22957-022 &        4379.230 &            0.58 &            0.30 \\ 
      CS~22957-022 &        4389.979 &            0.58 &            0.20 \\ 
      CS~22957-026 &        4379.230 &            2.05 &            0.10 \\ 
      CS~22957-026 &        4389.979 &            1.90 &            0.20 \\ 
      CS~22957-036 &        4379.230 &            1.79 &            0.30 \\ 
      CS~22958-037 &        4379.230 &            1.54 &            0.10 \\ 
      CS~22958-065 &        4379.230 &            1.71 &            0.15 \\ 
      CS~22958-083 &        4111.779 &            1.03 &            0.30 \\ 
      CS~22958-083 &        4379.230 &            0.79 &            0.06 \\ 
      CS~22958-083 &        4389.979 &            0.67 &            0.20 \\ 
      CS~22959-074 &        4111.779 &            1.17 &            0.15 \\ 
      CS~22959-074 &        4379.230 &            1.05 &            0.10 \\ 
      CS~22959-074 &        4389.979 &            1.02 &            0.06 \\ 
      CS~22959-074 &        4408.196 &            0.90 &            0.20 \\ 
      CS~22960-010 &        4379.230 &            0.70 &            0.06 \\ 
      CS~22960-048 &        4111.779 &            0.53 &            0.20 \\ 
      CS~22960-064 &        4111.779 &            1.02 &            0.10 \\ 
      CS~22960-064 &        4379.230 &            0.99 &            0.06 \\ 
      CS~22960-064 &        4389.979 &            1.11 &            0.20 \\ 
      CS~22965-016 &        4111.779 &            0.85 &            0.10 \\ 
      CS~22965-016 &        4379.230 &            0.85 &            0.10 \\ 
      CS~22965-016 &        4389.979 &            0.64 &            0.10 \\ 
      CS~22968-014 &        4379.230 &           -0.03 &            0.20 \\ 
      CS~22968-026 &        4111.779 &            1.45 &            0.20 \\ 
      CS~22968-026 &        4379.230 &            1.30 &            0.20 \\ 
      CS~29493-062 &        4379.230 &            1.25 &            0.30 \\ 
      CS~29495-005 &        4379.230 &            1.57 &            0.10 \\ 
      CS~29513-003 &        4111.779 &            1.59 &            0.05 \\ 
      CS~29513-003 &        4379.230 &            1.35 &            0.10 \\ 
      CS~29513-014 &        4111.779 &            1.59 &            0.10 \\ 
      CS~29513-014 &        4379.230 &            1.62 &            0.10 \\ 
      CS~29513-032 &        4379.230 &            2.05 &            0.10 \\ 
      CS~29514-017 &        4111.779 &            1.22 &            0.30 \\ 
      CS~29514-017 &        4379.230 &            1.28 &            0.10 \\ 
      CS~29514-017 &        4389.979 &            1.52 &            0.20 \\ 
      CS~29514-037 &        4379.230 &            1.66 &            0.06 \\ 
      CS~29517-018 &        4379.230 &            1.29 &            0.15 \\ 
      CS~29529-054 &        4379.230 &            1.35 &            0.10 \\ 
      CS~30312-044 &        4111.779 &            0.67 &            0.20 \\ 
      CS~30312-044 &        4379.230 &            0.58 &            0.06 \\ 
      CS~30312-044 &        4389.979 &            0.73 &            0.30 \\ 
      CS~30312-059 &        4111.779 &            0.30 &            0.10 \\ 
      CS~30312-059 &        4379.230 &            0.33 &            0.10 \\ 
      CS~30312-059 &        4389.979 &            0.27 &            0.10 \\ 
      CS~30312-100 &        4111.779 &            1.22 &            0.10 \\ 
      CS~30312-100 &        4379.230 &            1.19 &            0.06 \\ 
      CS~30312-100 &        4389.979 &            1.16 &            0.30 \\ 
      CS~30314-067 &        4111.779 &            0.20 &            0.20 \\ 
      CS~30314-067 &        4379.230 &            0.14 &            0.10 \\ 
      CS~30314-067 &        4389.979 &            0.38 &            0.20 \\ 
      CS~30492-001 &        4379.230 &            1.46 &            0.15 \\ 
      CS~30492-110 &        4379.230 &            0.33 &            0.20 \\ 
      CS~30493-071 &        4379.230 &            1.29 &            0.06 \\ 
      CS~30494-003 &        4111.779 &            0.75 &            0.10 \\ 
      CS~30494-003 &        4379.230 &            0.75 &            0.06 \\ 
      CS~30494-003 &        4389.979 &            0.81 &            0.30 \\ 
      CS~31082-001 &        4111.779 &            0.51 &            0.15 \\ 
      CS~31082-001 &        4379.230 &            0.69 &            0.06 \\ 
      CS~31082-001 &        4389.979 &            0.81 &            0.06 \\ 
         G~004-036 &        4111.779 &            2.06 &            0.20 \\ 
         G~004-036 &        4379.230 &            1.91 &            0.06 \\ 
         G~009-027 &        4111.779 &            1.91 &            0.30 \\ 
         G~009-027 &        4379.230 &            1.91 &            0.20 \\ 
         G~010-054 &        4379.230 &            1.42 &            0.15 \\ 
         G~010-054 &        4389.979 &            1.63 &            0.10 \\ 
         G~015-010 &        4111.779 &            1.26 &            0.10 \\ 
         G~015-010 &        4379.230 &            1.23 &            0.06 \\ 
         G~015-010 &        4389.979 &            1.20 &            0.10 \\ 
         G~016-025 &        4111.779 &            1.66 &            0.25 \\ 
         G~016-025 &        4379.230 &            1.51 &            0.10 \\ 
         G~025-022 &        4379.230 &            1.58 &            0.20 \\ 
         G~025-022 &        4389.979 &            1.34 &            0.20 \\ 
         G~025-024 &        4379.230 &            1.73 &            0.15 \\ 
         G~026-001 &        4111.779 &            1.95 &            0.10 \\ 
         G~026-001 &        4379.230 &            1.71 &            0.15 \\ 
         G~071-055 &        4111.779 &            1.83 &            0.10 \\ 
         G~071-055 &        4379.230 &            1.68 &            0.10 \\ 
         G~071-055 &        4389.979 &            1.59 &            0.10 \\ 
         G~071-055 &        4408.196 &            1.83 &            0.20 \\ 
         G~088-023 &        4111.779 &            2.09 &            0.30 \\ 
         G~088-023 &        4379.230 &            1.85 &            0.15 \\ 
         G~088-023 &        4389.979 &            1.70 &            0.10 \\ 
         G~088-023 &        4408.196 &            2.00 &            0.10 \\ 
         G~090-003 &        4111.779 &            1.54 &            0.15 \\ 
         G~090-003 &        4379.230 &            1.51 &            0.06 \\ 
         G~090-003 &        4389.979 &            1.54 &            0.15 \\ 
         G~090-025 &        4111.779 &            1.81 &            0.10 \\ 
         G~090-025 &        4379.230 &            1.78 &            0.10 \\ 
         G~090-025 &        4389.979 &            1.57 &            0.30 \\ 
         G~115-049 &        4379.230 &            1.25 &            0.15 \\ 
         G~126-062 &        4111.779 &            2.20 &            0.10 \\ 
         G~126-062 &        4379.230 &            2.17 &            0.06 \\ 
         G~126-062 &        4389.979 &            1.96 &            0.10 \\ 
         G~126-062 &        4408.196 &            2.17 &            0.05 \\ 
         G~137-086 &        4379.230 &            1.92 &            0.15 \\ 
         G~146-056 &        4111.779 &            2.30 &            0.05 \\ 
         G~146-056 &        4379.230 &            2.33 &            0.06 \\ 
         G~146-056 &        4389.979 &            2.03 &            0.10 \\ 
         G~146-056 &        4408.196 &            2.00 &            0.10 \\ 
         G~146-076 &        4111.779 &            1.67 &            0.10 \\ 
         G~146-076 &        4379.230 &            1.76 &            0.30 \\ 
         G~146-076 &        4389.979 &            1.46 &            0.10 \\ 
         G~153-064 &        4111.779 &            2.76 &            0.10 \\ 
         G~153-064 &        4379.230 &            2.70 &            0.10 \\ 
         G~153-064 &        4389.979 &            2.70 &            0.20 \\ 
         G~161-073 &        4111.779 &            2.28 &            0.10 \\ 
         G~161-073 &        4379.230 &            2.25 &            0.06 \\ 
         G~161-073 &        4389.979 &            2.16 &            0.10 \\ 
         G~170-047 &        4111.779 &            0.86 &            0.10 \\ 
         G~170-047 &        4379.230 &            0.80 &            0.10 \\ 
         G~170-047 &        4389.979 &            0.65 &            0.20 \\ 
         G~180-058 &        4111.779 &            1.39 &            0.20 \\ 
         G~180-058 &        4379.230 &            1.39 &            0.10 \\ 
         G~188-022 &        4111.779 &            2.31 &            0.10 \\ 
         G~188-022 &        4379.230 &            2.37 &            0.10 \\ 
         G~188-022 &        4389.979 &            2.16 &            0.10 \\ 
         G~188-022 &        4408.196 &            2.19 &            0.05 \\ 
         G~188-030 &        4111.779 &            1.81 &            0.10 \\ 
         G~188-030 &        4379.230 &            2.08 &            0.20 \\ 
         G~188-030 &        4389.979 &            1.78 &            0.20 \\ 
         G~190-010 &        4111.779 &            1.95 &            0.10 \\ 
         G~190-010 &        4379.230 &            1.71 &            0.20 \\ 
         G~190-010 &        4389.979 &            1.65 &            0.10 \\ 
         G~190-010 &        4408.196 &            1.74 &            0.10 \\ 
         G~190-015 &        4111.779 &            0.77 &            0.10 \\ 
         G~190-015 &        4379.230 &            0.77 &            0.15 \\ 
         G~199-066 &        4379.230 &            1.64 &            0.15 \\ 
         G~199-066 &        4389.979 &            1.64 &            0.10 \\ 
         G~201-044 &        4111.779 &            2.27 &            0.10 \\ 
         G~201-044 &        4379.230 &            2.12 &            0.20 \\ 
         G~214-001 &        4111.779 &            1.93 &            0.20 \\ 
         G~214-001 &        4379.230 &            1.42 &            0.10 \\ 
         G~234-028 &        4111.779 &            2.00 &            0.20 \\ 
         G~234-028 &        4379.230 &            1.94 &            0.10 \\ 
         G~238-032 &        4111.779 &            2.24 &            0.10 \\ 
         G~238-032 &        4379.230 &            2.24 &            0.10 \\ 
         G~238-032 &        4389.979 &            2.18 &            0.10 \\ 
         G~238-032 &        4408.196 &            2.06 &            0.20 \\ 
         HD~108317 &        4111.779 &            1.27 &            0.05 \\ 
         HD~108317 &        4111.779 &            1.27 &            0.30 \\ 
         HD~108317 &        4379.230 &            1.00 &            0.10 \\ 
         HD~108317 &        4379.230 &            1.21 &            0.10 \\ 
         HD~108317 &        4389.979 &            1.03 &            0.10 \\ 
         HD~108317 &        4389.979 &            1.12 &            0.20 \\ 
         HD~108317 &        4408.196 &            0.97 &            0.10 \\ 
          HD~11582 &        4111.779 &            1.77 &            0.05 \\ 
          HD~11582 &        4379.230 &            1.80 &            0.06 \\ 
          HD~11582 &        4389.979 &            1.95 &            0.10 \\ 
          HD~11582 &        4408.196 &            1.74 &            0.05 \\ 
         HD~119516 &        4111.779 &            1.86 &            0.10 \\ 
         HD~119516 &        4379.230 &            1.86 &            0.10 \\ 
         HD~119516 &        4389.979 &            1.65 &            0.20 \\ 
         HD~119516 &        4408.196 &            1.65 &            0.20 \\ 
         HD~122196 &        4379.230 &            1.83 &            0.20 \\ 
         HD~122563 &        4111.779 &            0.71 &            0.05 \\ 
         HD~122563 &        4111.779 &            0.77 &            0.10 \\ 
         HD~122563 &        4111.779 &            0.77 &            0.10 \\ 
         HD~122563 &        4379.230 &            0.68 &            0.06 \\ 
         HD~122563 &        4379.230 &            0.71 &            0.06 \\ 
         HD~122563 &        4379.230 &            0.71 &            0.06 \\ 
         HD~122563 &        4389.979 &            0.62 &            0.30 \\ 
         HD~122563 &        4389.979 &            0.77 &            0.15 \\ 
         HD~122563 &        4389.979 &            0.80 &            0.06 \\ 
         HD~122563 &        4408.196 &            0.56 &            0.10 \\ 
         HD~122563 &        4408.196 &            0.62 &            0.15 \\ 
         HD~122563 &        4408.196 &            0.80 &            0.20 \\ 
         HD~126238 &        4111.779 &            1.50 &            0.05 \\ 
         HD~126238 &        4379.230 &            1.47 &            0.06 \\ 
         HD~126238 &        4389.979 &            1.47 &            0.10 \\ 
         HD~126587 &        4111.779 &            0.53 &            0.05 \\ 
         HD~126587 &        4379.230 &            0.53 &            0.06 \\ 
         HD~126587 &        4389.979 &            0.53 &            0.15 \\ 
         HD~128279 &        4111.779 &            1.31 &            0.05 \\ 
         HD~128279 &        4379.230 &            1.28 &            0.06 \\ 
         HD~128279 &        4389.979 &            1.31 &            0.10 \\ 
         HD~132475 &        4111.779 &            2.01 &            0.05 \\ 
         HD~132475 &        4111.779 &            2.01 &            0.05 \\ 
         HD~132475 &        4379.230 &            1.89 &            0.06 \\ 
         HD~132475 &        4379.230 &            1.95 &            0.06 \\ 
         HD~132475 &        4389.979 &            1.95 &            0.15 \\ 
         HD~132475 &        4389.979 &            1.95 &            0.15 \\ 
         HD~132475 &        4408.196 &            1.80 &            0.10 \\ 
         HD~132475 &        4408.196 &            1.80 &            0.20 \\ 
          HD~13979 &        4111.779 &            0.81 &            0.05 \\ 
          HD~13979 &        4379.230 &            0.78 &            0.06 \\ 
          HD~13979 &        4389.979 &            0.79 &            0.10 \\ 
          HD~13979 &        4408.196 &            0.84 &            0.30 \\ 
          HD~16031 &        4111.779 &            1.86 &            0.10 \\ 
          HD~16031 &        4379.230 &            1.86 &            0.10 \\ 
         HD~175305 &        4111.779 &            2.03 &            0.10 \\ 
         HD~175305 &        4379.230 &            1.90 &            0.10 \\ 
         HD~175305 &        4389.979 &            1.88 &            0.10 \\ 
         HD~175305 &        4408.196 &            1.88 &            0.10 \\ 
         HD~175606 &        4111.779 &            1.54 &            0.30 \\ 
         HD~175606 &        4379.230 &            1.54 &            0.30 \\ 
         HD~178443 &        4111.779 &            1.83 &            0.05 \\ 
         HD~178443 &        4379.230 &            1.83 &            0.06 \\ 
         HD~178443 &        4389.979 &            1.83 &            0.06 \\ 
         HD~178443 &        4408.196 &            1.89 &            0.20 \\ 
         HD~184266 &        4111.779 &            2.15 &            0.10 \\ 
         HD~184266 &        4379.230 &            2.12 &            0.10 \\ 
         HD~184266 &        4408.196 &            2.42 &            0.20 \\ 
         HD~186478 &        4111.779 &            0.88 &            0.10 \\ 
         HD~186478 &        4379.230 &            0.88 &            0.06 \\ 
         HD~186478 &        4389.979 &            0.94 &            0.06 \\ 
         HD~186478 &        4408.196 &            0.73 &            0.10 \\ 
         HD~188510 &        4111.779 &            1.87 &            0.10 \\ 
         HD~188510 &        4379.230 &            1.84 &            0.10 \\ 
         HD~188510 &        4389.979 &            1.81 &            0.20 \\ 
         HD~193901 &        4111.779 &            2.47 &            0.10 \\ 
         HD~193901 &        4379.230 &            2.32 &            0.10 \\ 
         HD~193901 &        4389.979 &            2.42 &            0.10 \\ 
         HD~193901 &        4408.196 &            2.26 &            0.15 \\ 
          HD~19445 &        4111.779 &            1.67 &            0.15 \\ 
         HD~196892 &        4111.779 &            2.47 &            0.10 \\ 
         HD~196892 &        4379.230 &            2.47 &            0.06 \\ 
         HD~196892 &        4389.979 &            2.38 &            0.10 \\ 
         HD~196944 &        4111.779 &            1.22 &            0.30 \\ 
         HD~196944 &        4389.979 &            1.49 &            0.10 \\ 
         HD~200654 &        4111.779 &            0.76 &            0.05 \\ 
         HD~200654 &        4379.230 &            0.79 &            0.06 \\ 
         HD~200654 &        4389.979 &            1.06 &            0.30 \\ 
         HD~201891 &        4111.779 &            2.71 &            0.10 \\ 
         HD~201891 &        4379.230 &            2.59 &            0.10 \\ 
         HD~201891 &        4389.979 &            2.62 &            0.30 \\ 
         HD~201891 &        4408.196 &            2.47 &            0.10 \\ 
         HD~214362 &        4111.779 &            1.67 &            0.20 \\ 
         HD~214362 &        4379.230 &            1.82 &            0.06 \\ 
         HD~214362 &        4389.979 &            1.52 &            0.10 \\ 
          HD~21581 &        4111.779 &            1.98 &            0.10 \\ 
          HD~21581 &        4379.230 &            2.01 &            0.10 \\ 
          HD~21581 &        4389.979 &            2.04 &            0.10 \\ 
         HD~219617 &        4111.779 &            2.31 &            0.20 \\ 
         HD~219617 &        4379.230 &            2.13 &            0.06 \\ 
         HD~219617 &        4389.979 &            2.01 &            0.10 \\ 
         HD~219617 &        4408.196 &            2.10 &            0.30 \\ 
         HD~220127 &        4111.779 &            2.00 &            0.05 \\ 
         HD~220127 &        4379.230 &            2.00 &            0.10 \\ 
         HD~220127 &        4389.979 &            1.97 &            0.06 \\ 
         HD~237846 &        4379.230 &            0.43 &            0.10 \\ 
          HD~26169 &        4111.779 &            1.03 &            0.10 \\ 
          HD~26169 &        4379.230 &            1.03 &            0.10 \\ 
          HD~26169 &        4389.979 &            1.03 &            0.30 \\ 
          HD~26297 &        4111.779 &            1.59 &            0.20 \\ 
          HD~26297 &        4379.230 &            1.50 &            0.20 \\ 
          HD~26297 &        4389.979 &            1.40 &            0.30 \\ 
          HD~26297 &        4408.196 &            1.50 &            0.10 \\ 
          HD~31128 &        4111.779 &            1.91 &            0.05 \\ 
          HD~31128 &        4379.230 &            1.94 &            0.06 \\ 
          HD~31128 &        4389.979 &            1.79 &            0.20 \\ 
          HD~31128 &        4408.196 &            1.64 &            0.20 \\ 
          HD~45282 &        4111.779 &            2.12 &            0.05 \\ 
          HD~45282 &        4379.230 &            2.12 &            0.10 \\ 
          HD~45282 &        4389.979 &            2.06 &            0.10 \\ 
          HD~45282 &        4408.196 &            2.06 &            0.10 \\ 
           HD~6268 &        4111.779 &            0.74 &            0.10 \\ 
           HD~6268 &        4379.230 &            0.86 &            0.10 \\ 
           HD~6268 &        4389.979 &            0.80 &            0.20 \\ 
           HD~6268 &        4408.196 &            0.83 &            0.15 \\ 
          HD~88609 &        4111.779 &            0.30 &            0.10 \\ 
          HD~88609 &        4379.230 &            0.24 &            0.10 \\ 
          HD~88609 &        4408.196 &            0.30 &            0.30 \\ 
          HD~94028 &        4111.779 &            2.05 &            0.10 \\ 
          HD~94028 &        4379.230 &            2.08 &            0.10 \\ 
      HE~0454$-$4758 &        4111.779 &            0.94 &            0.30 \\ 
      HE~0454$-$4758 &        4379.230 &            0.64 &            0.30 \\ 
      HE~1124$-$2335 &        4379.230 &            0.36 &            0.15 \\ 
      HE~1320$-$1339 &        4111.779 &            0.67 &            0.10 \\ 
      HE~1320$-$1339 &        4111.779 &            0.70 &            0.10 \\ 
      HE~1320$-$1339 &        4379.230 &            0.64 &            0.06 \\ 
      HE~1320$-$1339 &        4379.230 &            0.67 &            0.06 \\ 
      HE~1320$-$1339 &        4389.979 &            0.70 &            0.10 \\ 
      HE~1320$-$1339 &        4389.979 &            0.70 &            0.30 \\ 
      HE~1320$-$1339 &        4408.196 &            0.70 &            0.10 \\ 
      HE~1320$-$1339 &        4408.196 &            0.85 &            0.20 \\ 
         HIP~99423 &        4111.779 &            2.06 &            0.05 \\ 
         HIP~99423 &        4379.230 &            2.06 &            0.06 \\ 
         HIP~99423 &        4389.979 &            2.03 &            0.10 \\ 
         HIP~99423 &        4408.196 &            2.03 &            0.10 \\ 
\enddata      
\tablecomments{%
The model atmosphere uncertainty is not included in here for reasons 
discussed in Section~\ref{uncertainties}
}
\end{deluxetable}

==> tab03.tex <==
\startlongtable
\begin{deluxetable}{cccc}
\tablecaption{Abundances Derived from Ionized Vanadium Lines
\label{v2tab}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Star} &
\colhead{Wavelength (\AA)} &
\colhead{\log \epsilon (V~\textsc{ii})} &
\colhead{$\sigma$}
}
\startdata
      BD~$+$10\degree2495 &        3715.464 &            1.70 &            0.17 \\ 
      BD~$+$10\degree2495 &        3951.957 &            1.77 &            0.18 \\ 
      BD~$+$10\degree2495 &        4002.928 &            1.69 &            0.11 \\ 
      BD~$+$10\degree2495 &        4005.702 &            1.87 &            0.15 \\ 
      BD~$+$10\degree2495 &        4023.377 &            1.87 &            0.11 \\ 
     BD~$+$19\degree1185a &        3715.464 &            2.74 &            0.18 \\ 
     BD~$+$19\degree1185a &        3951.957 &            2.76 &            0.14 \\ 
     BD~$+$19\degree1185a &        4002.928 &            2.71 &            0.20 \\ 
     BD~$+$19\degree1185a &        4005.702 &            2.86 &            0.06 \\ 
      BD~$+$24\degree1676 &        3715.464 &            1.54 &            0.34 \\ 
      BD~$+$24\degree1676 &        3951.957 &            1.46 &            0.22 \\ 
      BD~$+$24\degree1676 &        4005.702 &            1.74 &            0.06 \\ 
      BD~$+$26\degree3578 &        3951.957 &            1.78 &            0.51 \\ 
      BD~$+$26\degree3578 &        4005.702 &            1.73 &            0.30 \\ 
      BD~$+$29\degree2356 &        3951.957 &            2.31 &            0.22 \\ 
      BD~$+$29\degree2356 &        4002.928 &            2.51 &            0.20 \\ 
      BD~$+$29\degree2356 &        4005.702 &            2.51 &            0.15 \\ 
      BD~$+$29\degree2356 &        4023.377 &            2.47 &            0.15 \\ 
      BD~$+$80\degree0245 &        3951.957 &            1.51 &            0.14 \\ 
      BD~$+$80\degree0245 &        4005.702 &            1.43 &            0.30 \\ 
      BD~$+$80\degree0245 &        4023.377 &            1.58 &            0.15 \\ 
      BD~$-$01\degree2582 &        3715.464 &            1.35 &            0.17 \\ 
      BD~$-$01\degree2582 &        3951.957 &            1.41 &            0.18 \\ 
      BD~$-$01\degree2582 &        4002.928 &            1.37 &            0.11 \\ 
      BD~$-$01\degree2582 &        4005.702 &            1.31 &            0.06 \\ 
      BD~$-$01\degree2582 &        4023.377 &            1.25 &            0.06 \\ 
     BD~$-$15\degree5781 &        3517.299 &            1.07 &            0.12 \\ 
     BD~$-$15\degree5781 &        3545.196 &            0.99 &            0.11 \\ 
     BD~$-$15\degree5781 &        3715.464 &            0.85 &            0.17 \\ 
     BD~$-$15\degree5781 &        3951.957 &            1.02 &            0.14 \\ 
     BD~$-$15\degree5781 &        4002.928 &            0.94 &            0.11 \\ 
     BD~$-$15\degree5781 &        4005.702 &            0.97 &            0.11 \\ 
     BD~$-$15\degree5781 &        4023.377 &            1.02 &            0.06 \\ 
      BD~$-$18\degree5550 &        3715.464 &            0.69 &            0.24 \\ 
      BD~$-$18\degree5550 &        3951.957 &            0.74 &            0.14 \\ 
      BD~$-$18\degree5550 &        4002.928 &            0.92 &            0.11 \\ 
      BD~$-$18\degree5550 &        4005.702 &            0.86 &            0.11 \\ 
      BD~$-$18\degree5550 &        4023.377 &            0.77 &            0.15 \\ 
     BD~$-$20\degree6008 &        3517.299 &            0.93 &            0.31 \\ 
     BD~$-$20\degree6008 &        3545.196 &            1.21 &            0.30 \\ 
     BD~$-$20\degree6008 &        3715.464 &            0.74 &            0.17 \\ 
     BD~$-$20\degree6008 &        3951.957 &            1.21 &            0.14 \\ 
     BD~$-$20\degree6008 &        4002.928 &            0.82 &            0.11 \\ 
     BD~$-$20\degree6008 &        4005.702 &            0.88 &            0.11 \\ 
     BD~$-$20\degree6008 &        4023.377 &            0.97 &            0.11 \\ 
     CD~$-$24\degree1782 &        3517.299 &            1.21 &            0.17 \\ 
     CD~$-$24\degree1782 &        3545.196 &            0.91 &            0.16 \\ 
     CD~$-$24\degree1782 &        3715.464 &            0.83 &            0.17 \\ 
     CD~$-$24\degree1782 &        4002.928 &            1.00 &            0.15 \\ 
     CD~$-$24\degree1782 &        4005.702 &            1.09 &            0.06 \\ 
     CD~$-$24\degree1782 &        4023.377 &            1.09 &            0.15 \\ 
     CD~$-$30\degree0298 &        3517.299 &            0.22 &            0.31 \\ 
     CD~$-$30\degree0298 &        3545.196 &            0.20 &            0.40 \\ 
     CD~$-$30\degree0298 &        3715.464 &            0.41 &            0.24 \\ 
     CD~$-$30\degree0298 &        4005.702 &            0.10 &            0.20 \\ 
     CD~$-$36\degree1052 &        3517.299 &            2.27 &            0.17 \\ 
     CD~$-$36\degree1052 &        3545.196 &            2.38 &            0.21 \\ 
     CD~$-$36\degree1052 &        3715.464 &            2.15 &            0.19 \\ 
     CD~$-$36\degree1052 &        3951.957 &            2.22 &            0.18 \\ 
     CD~$-$36\degree1052 &        4002.928 &            2.10 &            0.11 \\ 
     CD~$-$36\degree1052 &        4005.702 &            2.18 &            0.06 \\ 
     CD~$-$36\degree1052 &        4023.377 &            2.04 &            0.06 \\ 
      CS~22166-016 &        3517.299 &            0.92 &            0.13 \\ 
      CS~22166-016 &        3545.196 &            0.89 &            0.11 \\ 
      CS~22166-016 &        3715.464 &            0.93 &            0.17 \\ 
      CS~22166-016 &        3951.957 &            1.05 &            0.14 \\ 
      CS~22166-016 &        4002.928 &            1.04 &            0.30 \\ 
      CS~22166-016 &        4005.702 &            0.95 &            0.20 \\ 
      CS~22166-016 &        4023.377 &            1.04 &            0.20 \\ 
      CS~22169-008 &        3517.299 &            1.64 &            0.22 \\ 
      CS~22169-008 &        3545.196 &            1.51 &            0.21 \\ 
      CS~22169-008 &        3715.464 &            1.51 &            0.25 \\ 
      CS~22169-008 &        4005.702 &            1.46 &            0.30 \\ 
      CS~22169-008 &        4023.377 &            1.49 &            0.15 \\ 
      CS~22169-035 &        3517.299 &            0.40 &            0.31 \\ 
      CS~22169-035 &        3715.464 &            0.57 &            0.33 \\ 
      CS~22169-035 &        3951.957 &            0.14 &            0.13 \\ 
      CS~22169-035 &        4005.702 &            0.44 &            0.20 \\ 
      CS~22169-035 &        4023.377 &            0.59 &            0.30 \\ 
      CS~22171-031 &        3517.299 &            1.80 &            0.22 \\ 
      CS~22171-031 &        3545.196 &            1.91 &            0.11 \\ 
      CS~22171-031 &        3715.464 &            1.98 &            0.19 \\ 
      CS~22171-031 &        3951.957 &            1.87 &            0.22 \\ 
      CS~22171-031 &        4005.702 &            1.66 &            0.30 \\ 
      CS~22171-031 &        4023.377 &            1.51 &            0.40 \\ 
      CS~22172-029 &        3517.299 &            1.28 &            0.13 \\ 
      CS~22172-029 &        3545.196 &            1.56 &            0.07 \\ 
      CS~22172-029 &        3715.464 &            1.24 &            0.15 \\ 
      CS~22172-029 &        3951.957 &            1.39 &            0.11 \\ 
      CS~22172-029 &        4002.928 &            1.35 &            0.11 \\ 
      CS~22172-029 &        4005.702 &            1.26 &            0.06 \\ 
      CS~22172-029 &        4023.377 &            1.32 &            0.06 \\ 
      CS~22174-020 &        3517.299 &            1.56 &            0.31 \\ 
      CS~22177-009 &        4023.377 &            1.25 &            0.30 \\ 
      CS~22177-010 &        3517.299 &            1.28 &            0.22 \\ 
      CS~22180-014 &        3517.299 &            1.15 &            0.22 \\ 
      CS~22180-014 &        3715.464 &            1.42 &            0.25 \\ 
      CS~22182-033 &        3517.299 &            1.80 &            0.22 \\ 
      CS~22182-033 &        3545.196 &            1.46 &            0.21 \\ 
      CS~22182-033 &        3951.957 &            1.65 &            0.14 \\ 
      CS~22182-033 &        4023.377 &            1.68 &            0.11 \\ 
      CS~22182-047 &        3517.299 &            1.98 &            0.09 \\ 
      CS~22182-047 &        3545.196 &            1.95 &            0.07 \\ 
      CS~22182-047 &        3715.464 &            1.93 &            0.16 \\ 
      CS~22182-047 &        3951.957 &            2.10 &            0.11 \\ 
      CS~22182-047 &        4002.928 &            2.03 &            0.20 \\ 
      CS~22182-047 &        4005.702 &            1.94 &            0.06 \\ 
      CS~22182-047 &        4023.377 &            2.06 &            0.06 \\ 
      CS~22183-031 &        3517.299 &            0.70 &            0.13 \\ 
      CS~22183-031 &        3545.196 &            0.71 &            0.11 \\ 
      CS~22183-031 &        3715.464 &            0.68 &            0.17 \\ 
      CS~22183-031 &        3951.957 &            0.72 &            0.14 \\ 
      CS~22183-031 &        4023.377 &            0.64 &            0.11 \\ 
      CS~22185-007 &        3517.299 &            1.35 &            0.31 \\ 
      CS~22185-007 &        3545.196 &            1.18 &            0.21 \\ 
      CS~22185-007 &        3715.464 &            1.17 &            0.17 \\ 
      CS~22185-007 &        3951.957 &            1.00 &            0.14 \\ 
      CS~22185-007 &        4002.928 &            1.19 &            0.20 \\ 
      CS~22185-007 &        4005.702 &            1.01 &            0.11 \\ 
      CS~22185-007 &        4023.377 &            1.07 &            0.06 \\ 
      CS~22186-002 &        3517.299 &            1.55 &            0.09 \\ 
      CS~22186-002 &        3545.196 &            1.40 &            0.07 \\ 
      CS~22186-002 &        3715.464 &            1.50 &            0.18 \\ 
      CS~22186-002 &        3951.957 &            1.52 &            0.14 \\ 
      CS~22186-002 &        4005.702 &            1.38 &            0.11 \\ 
      CS~22186-002 &        4023.377 &            1.23 &            0.11 \\ 
      CS~22186-017 &        3715.464 &            1.35 &            0.25 \\ 
      CS~22186-017 &        4005.702 &            1.48 &            0.15 \\ 
      CS~22186-023 &        3517.299 &            1.10 &            0.13 \\ 
      CS~22186-023 &        3545.196 &            1.23 &            0.21 \\ 
      CS~22186-023 &        3715.464 &            1.02 &            0.15 \\ 
      CS~22186-023 &        3951.957 &            0.97 &            0.14 \\ 
      CS~22186-023 &        4002.928 &            0.95 &            0.20 \\ 
      CS~22186-023 &        4005.702 &            1.07 &            0.11 \\ 
      CS~22186-023 &        4023.377 &            1.22 &            0.20 \\ 
      CS~22189-009 &        3517.299 &            0.09 &            0.12 \\ 
      CS~22189-009 &        3545.196 &           -0.08 &            0.11 \\ 
      CS~22189-009 &        3715.464 &            0.17 &            0.17 \\ 
      CS~22189-009 &        3951.957 &           -0.20 &            0.22 \\ 
      CS~22189-009 &        4005.702 &            0.04 &            0.20 \\ 
      CS~22189-009 &        4023.377 &            0.07 &            0.20 \\ 
      CS~22191-029 &        3715.464 &            1.25 &            0.25 \\ 
      CS~22191-029 &        3951.957 &            1.11 &            0.14 \\ 
      CS~22191-029 &        4005.702 &            1.11 &            0.11 \\ 
      CS~22191-029 &        4023.377 &            1.20 &            0.11 \\ 
      CS~22873-128 &        3517.299 &            0.73 &            0.09 \\ 
      CS~22873-128 &        3545.196 &            0.89 &            0.07 \\ 
      CS~22873-128 &        3715.464 &            0.94 &            0.15 \\ 
      CS~22873-128 &        3951.957 &            1.01 &            0.10 \\ 
      CS~22873-128 &        4005.702 &            0.87 &            0.06 \\ 
      CS~22873-128 &        4023.377 &            0.93 &            0.11 \\ 
      CS~22875-029 &        3715.464 &            1.51 &            0.25 \\ 
      CS~22875-029 &        3951.957 &            1.43 &            0.14 \\ 
      CS~22875-029 &        4002.928 &            1.67 &            0.20 \\ 
      CS~22875-029 &        4005.702 &            1.43 &            0.11 \\ 
      CS~22875-029 &        4023.377 &            1.49 &            0.06 \\ 
      CS~22876-040 &        3517.299 &            1.84 &            0.22 \\ 
      CS~22876-040 &        3951.957 &            1.81 &            0.14 \\ 
      CS~22876-040 &        4005.702 &            1.94 &            0.11 \\ 
      CS~22876-040 &        4023.377 &            1.91 &            0.11 \\ 
      CS~22877-001 &        3517.299 &            0.59 &            0.13 \\ 
      CS~22877-001 &        3545.196 &            0.66 &            0.11 \\ 
      CS~22877-001 &        3715.464 &            0.57 &            0.17 \\ 
      CS~22877-001 &        3951.957 &            0.61 &            0.18 \\ 
      CS~22877-001 &        4005.702 &            0.56 &            0.06 \\ 
      CS~22877-001 &        4023.377 &            0.41 &            0.11 \\ 
      CS~22877-011 &        3517.299 &            0.83 &            0.09 \\ 
      CS~22877-011 &        3545.196 &            0.86 &            0.30 \\ 
      CS~22877-011 &        3715.464 &            0.93 &            0.15 \\ 
      CS~22877-011 &        3951.957 &            0.84 &            0.11 \\ 
      CS~22877-011 &        4005.702 &            0.89 &            0.06 \\ 
      CS~22877-011 &        4023.377 &            0.80 &            0.20 \\ 
      CS~22877-015 &        3951.957 &            2.13 &            0.22 \\ 
      CS~22877-015 &        4005.702 &            2.23 &            0.06 \\ 
      CS~22877-015 &        4023.377 &            2.14 &            0.11 \\ 
      CS~22878-101 &        3517.299 &            0.52 &            0.12 \\ 
      CS~22878-101 &        3545.196 &            0.53 &            0.11 \\ 
      CS~22878-101 &        3715.464 &            0.79 &            0.17 \\ 
      CS~22878-101 &        3951.957 &            0.75 &            0.10 \\ 
      CS~22878-101 &        4002.928 &            0.96 &            0.30 \\ 
      CS~22878-101 &        4005.702 &            0.66 &            0.06 \\ 
      CS~22878-101 &        4023.377 &            0.66 &            0.20 \\ 
      CS~22879-029 &        3517.299 &            1.81 &            0.10 \\ 
      CS~22879-029 &        3545.196 &            1.59 &            0.21 \\ 
      CS~22879-029 &        3715.464 &            1.59 &            0.18 \\ 
      CS~22879-029 &        3951.957 &            1.51 &            0.22 \\ 
      CS~22879-029 &        4005.702 &            1.90 &            0.11 \\ 
      CS~22879-097 &        3517.299 &            1.29 &            0.31 \\ 
      CS~22879-097 &        3545.196 &            1.56 &            0.21 \\ 
      CS~22879-097 &        3715.464 &            1.42 &            0.18 \\ 
      CS~22879-097 &        3951.957 &            1.32 &            0.14 \\ 
      CS~22879-097 &        4002.928 &            1.40 &            0.30 \\ 
      CS~22879-097 &        4005.702 &            1.49 &            0.06 \\ 
      CS~22879-097 &        4023.377 &            1.46 &            0.11 \\ 
      CS~22879-103 &        3517.299 &            1.70 &            0.31 \\ 
      CS~22879-103 &        3545.196 &            1.81 &            0.21 \\ 
      CS~22879-103 &        3715.464 &            1.83 &            0.16 \\ 
      CS~22879-103 &        3951.957 &            1.88 &            0.11 \\ 
      CS~22879-103 &        4002.928 &            1.81 &            0.20 \\ 
      CS~22879-103 &        4005.702 &            1.96 &            0.11 \\ 
      CS~22879-103 &        4023.377 &            1.93 &            0.11 \\ 
      CS~22880-086 &        3517.299 &            0.97 &            0.31 \\ 
      CS~22880-086 &        3545.196 &            0.80 &            0.30 \\ 
      CS~22880-086 &        3715.464 &            0.90 &            0.25 \\ 
      CS~22880-086 &        3951.957 &            0.69 &            0.22 \\ 
      CS~22880-086 &        4005.702 &            0.89 &            0.11 \\ 
      CS~22880-086 &        4023.377 &            0.74 &            0.11 \\ 
      CS~22881-036 &        3517.299 &            2.01 &            0.13 \\ 
      CS~22881-036 &        3545.196 &            1.63 &            0.21 \\ 
      CS~22881-036 &        3715.464 &            1.58 &            0.34 \\ 
      CS~22881-036 &        3951.957 &            1.83 &            0.41 \\ 
      CS~22881-036 &        4005.702 &            1.65 &            0.20 \\ 
      CS~22881-039 &        4005.702 &            1.32 &            0.11 \\ 
      CS~22881-039 &        4023.377 &            1.53 &            0.30 \\ 
      CS~22881-070 &        3517.299 &            1.76 &            0.13 \\ 
      CS~22881-070 &        3545.196 &            1.48 &            0.21 \\ 
      CS~22881-070 &        3715.464 &            1.64 &            0.19 \\ 
      CS~22881-070 &        4005.702 &            1.32 &            0.20 \\ 
      CS~22882-001 &        3517.299 &            1.70 &            0.51 \\ 
      CS~22882-001 &        3545.196 &            1.59 &            0.30 \\ 
      CS~22882-001 &        3715.464 &            1.33 &            0.25 \\ 
      CS~22882-001 &        3951.957 &            1.58 &            0.14 \\ 
      CS~22882-001 &        4002.928 &            1.55 &            0.30 \\ 
      CS~22882-001 &        4005.702 &            1.67 &            0.20 \\ 
      CS~22882-001 &        4023.377 &            1.52 &            0.11 \\ 
      CS~22882-006 &        3517.299 &            1.46 &            0.13 \\ 
      CS~22882-006 &        3545.196 &            1.87 &            0.21 \\ 
      CS~22882-006 &        3715.464 &            1.63 &            0.34 \\ 
      CS~22882-006 &        3951.957 &            1.65 &            0.14 \\ 
      CS~22882-006 &        4023.377 &            1.43 &            0.20 \\ 
      CS~22883-037 &        3545.196 &            1.88 &            0.30 \\ 
      CS~22883-037 &        3715.464 &            1.85 &            0.18 \\ 
      CS~22883-037 &        3951.957 &            1.96 &            0.11 \\ 
      CS~22883-037 &        4002.928 &            1.89 &            0.11 \\ 
      CS~22883-037 &        4005.702 &            2.01 &            0.06 \\ 
      CS~22883-037 &        4023.377 &            2.19 &            0.11 \\ 
      CS~22884-020 &        3951.957 &            2.31 &            0.14 \\ 
      CS~22884-020 &        4002.928 &            2.14 &            0.11 \\ 
      CS~22884-020 &        4005.702 &            2.02 &            0.06 \\ 
      CS~22885-040 &        3951.957 &            1.79 &            0.22 \\ 
      CS~22885-040 &        4005.702 &            1.59 &            0.30 \\ 
      CS~22885-040 &        4023.377 &            1.44 &            0.20 \\ 
      CS~22885-096 &        3517.299 &            0.01 &            0.21 \\ 
      CS~22885-096 &        3545.196 &           -0.13 &            0.11 \\ 
      CS~22885-096 &        3715.464 &           -0.18 &            0.24 \\ 
      CS~22886-003 &        3517.299 &            1.82 &            0.31 \\ 
      CS~22886-003 &        4005.702 &            1.65 &            0.20 \\ 
      CS~22886-012 &        3517.299 &            1.97 &            0.13 \\ 
      CS~22886-012 &        3545.196 &            1.67 &            0.21 \\ 
      CS~22886-012 &        3951.957 &            1.67 &            0.22 \\ 
      CS~22886-012 &        4005.702 &            1.51 &            0.40 \\ 
      CS~22886-012 &        4023.377 &            1.54 &            0.20 \\ 
      CS~22886-013 &        3517.299 &            1.53 &            0.13 \\ 
      CS~22886-013 &        3545.196 &            1.45 &            0.11 \\ 
      CS~22886-013 &        3715.464 &            1.41 &            0.26 \\ 
      CS~22886-013 &        3951.957 &            1.39 &            0.32 \\ 
      CS~22886-013 &        4002.928 &            1.97 &            0.30 \\ 
      CS~22886-013 &        4005.702 &            1.82 &            0.30 \\ 
      CS~22886-013 &        4023.377 &            1.73 &            0.11 \\ 
      CS~22886-044 &        3517.299 &            2.34 &            0.41 \\ 
      CS~22886-044 &        3545.196 &            2.27 &            0.21 \\ 
      CS~22886-044 &        3715.464 &            2.41 &            0.34 \\ 
      CS~22886-044 &        3951.957 &            2.58 &            0.11 \\ 
      CS~22886-044 &        4002.928 &            2.15 &            0.30 \\ 
      CS~22886-044 &        4005.702 &            2.39 &            0.06 \\ 
      CS~22886-044 &        4023.377 &            2.33 &            0.11 \\ 
      CS~22888-002 &        3715.464 &            1.51 &            0.25 \\ 
      CS~22888-014 &        3517.299 &            1.46 &            0.22 \\ 
      CS~22888-014 &        3545.196 &            1.72 &            0.21 \\ 
      CS~22888-014 &        4005.702 &            1.59 &            0.20 \\ 
      CS~22888-047 &        3517.299 &            1.57 &            0.41 \\ 
      CS~22888-047 &        3545.196 &            1.67 &            0.40 \\ 
      CS~22888-047 &        3715.464 &            1.41 &            0.25 \\ 
      CS~22888-047 &        3951.957 &            1.36 &            0.14 \\ 
      CS~22888-047 &        4002.928 &            1.24 &            0.20 \\ 
      CS~22888-047 &        4005.702 &            1.42 &            0.11 \\ 
      CS~22888-047 &        4023.377 &            1.48 &            0.20 \\ 
      CS~22889-050 &        4005.702 &            1.48 &            0.30 \\ 
      CS~22889-050 &        4023.377 &            1.48 &            0.30 \\ 
      CS~22890-011 &        3545.196 &            1.83 &            0.16 \\ 
      CS~22890-011 &        3715.464 &            1.72 &            0.16 \\ 
      CS~22890-011 &        3951.957 &            1.61 &            0.32 \\ 
      CS~22890-011 &        4023.377 &            1.70 &            0.11 \\ 
      CS~22890-024 &        3517.299 &            1.33 &            0.13 \\ 
      CS~22890-024 &        3545.196 &            1.30 &            0.07 \\ 
      CS~22890-024 &        3715.464 &            1.48 &            0.18 \\ 
      CS~22890-024 &        3951.957 &            1.48 &            0.11 \\ 
      CS~22890-024 &        4005.702 &            1.36 &            0.20 \\ 
      CS~22890-024 &        4023.377 &            1.24 &            0.11 \\ 
      CS~22891-184 &        3517.299 &            1.01 &            0.22 \\ 
      CS~22891-184 &        3545.196 &            1.07 &            0.21 \\ 
      CS~22891-184 &        3715.464 &            1.25 &            0.18 \\ 
      CS~22891-184 &        3951.957 &            1.19 &            0.14 \\ 
      CS~22891-184 &        4005.702 &            1.11 &            0.11 \\ 
      CS~22891-184 &        4023.377 &            1.14 &            0.20 \\ 
      CS~22891-200 &        3545.196 &            0.05 &            0.11 \\ 
      CS~22891-200 &        3715.464 &           -0.16 &            0.24 \\ 
      CS~22891-200 &        4005.702 &            0.04 &            0.06 \\ 
      CS~22891-209 &        3517.299 &            0.61 &            0.12 \\ 
      CS~22891-209 &        3545.196 &            0.75 &            0.21 \\ 
      CS~22891-209 &        3715.464 &            0.82 &            0.15 \\ 
      CS~22891-209 &        3951.957 &            0.48 &            0.31 \\ 
      CS~22891-209 &        4002.928 &            0.78 &            0.20 \\ 
      CS~22891-209 &        4005.702 &            0.66 &            0.11 \\ 
      CS~22891-209 &        4023.377 &            0.90 &            0.11 \\ 
      CS~22892-025 &        3517.299 &            1.67 &            0.17 \\ 
      CS~22892-025 &        3545.196 &            1.78 &            0.30 \\ 
      CS~22892-025 &        4005.702 &            1.66 &            0.30 \\ 
      CS~22892-052 &        3517.299 &            0.57 &            0.09 \\ 
      CS~22892-052 &        3545.196 &            0.55 &            0.07 \\ 
      CS~22892-052 &        3715.464 &            0.60 &            0.20 \\ 
      CS~22892-052 &        3951.957 &            0.64 &            0.14 \\ 
      CS~22892-052 &        4002.928 &            0.62 &            0.06 \\ 
      CS~22892-052 &        4005.702 &            0.68 &            0.06 \\ 
      CS~22892-052 &        4023.377 &            0.62 &            0.06 \\ 
      CS~22893-005 &        3517.299 &            1.22 &            0.21 \\ 
      CS~22893-005 &        3715.464 &            1.39 &            0.21 \\ 
      CS~22893-005 &        4005.702 &            1.15 &            0.30 \\ 
      CS~22893-010 &        3545.196 &            1.26 &            0.40 \\ 
      CS~22893-010 &        3951.957 &            0.98 &            0.11 \\ 
      CS~22893-010 &        4005.702 &            1.22 &            0.11 \\ 
      CS~22893-011 &        3951.957 &            1.90 &            0.14 \\ 
      CS~22893-011 &        4005.702 &            1.96 &            0.15 \\ 
      CS~22893-011 &        4023.377 &            2.05 &            0.11 \\ 
      CS~22894-004 &        3951.957 &            1.94 &            0.22 \\ 
      CS~22894-019 &        3517.299 &            1.57 &            0.22 \\ 
      CS~22894-023 &        3517.299 &            1.35 &            0.13 \\ 
      CS~22894-023 &        3545.196 &            1.37 &            0.16 \\ 
      CS~22894-023 &        3715.464 &            1.26 &            0.25 \\ 
      CS~22894-023 &        4005.702 &            1.54 &            0.20 \\ 
      CS~22894-049 &        3545.196 &            1.55 &            0.21 \\ 
      CS~22896-015 &        3517.299 &            1.44 &            0.41 \\ 
      CS~22896-015 &        3545.196 &            0.96 &            0.30 \\ 
      CS~22896-015 &        3715.464 &            1.27 &            0.15 \\ 
      CS~22896-015 &        3951.957 &            1.04 &            0.11 \\ 
      CS~22896-015 &        4005.702 &            1.06 &            0.20 \\ 
      CS~22896-015 &        4023.377 &            1.21 &            0.20 \\ 
      CS~22896-055 &        3517.299 &            1.58 &            0.22 \\ 
      CS~22896-055 &        3545.196 &            1.69 &            0.30 \\ 
      CS~22896-055 &        3715.464 &            1.67 &            0.19 \\ 
      CS~22896-055 &        3951.957 &            1.71 &            0.14 \\ 
      CS~22896-055 &        4002.928 &            1.47 &            0.30 \\ 
      CS~22896-055 &        4005.702 &            1.59 &            0.06 \\ 
      CS~22896-055 &        4023.377 &            1.56 &            0.20 \\ 
      CS~22896-110 &        3517.299 &            1.21 &            0.31 \\ 
      CS~22896-110 &        3545.196 &            1.18 &            0.11 \\ 
      CS~22896-110 &        3715.464 &            1.42 &            0.18 \\ 
      CS~22896-110 &        3951.957 &            1.44 &            0.14 \\ 
      CS~22896-110 &        4005.702 &            1.21 &            0.11 \\ 
      CS~22896-110 &        4023.377 &            1.15 &            0.20 \\ 
      CS~22896-115 &        3545.196 &            1.51 &            0.21 \\ 
      CS~22896-115 &        3715.464 &            1.33 &            0.25 \\ 
      CS~22896-136 &        3517.299 &            1.74 &            0.31 \\ 
      CS~22896-136 &        3545.196 &            1.99 &            0.21 \\ 
      CS~22896-136 &        3715.464 &            1.92 &            0.17 \\ 
      CS~22896-136 &        3951.957 &            1.93 &            0.14 \\ 
      CS~22896-136 &        4005.702 &            1.97 &            0.06 \\ 
      CS~22897-008 &        3517.299 &            0.33 &            0.12 \\ 
      CS~22897-008 &        3545.196 &            0.46 &            0.21 \\ 
      CS~22897-008 &        3715.464 &            0.44 &            0.17 \\ 
      CS~22897-008 &        3951.957 &            0.46 &            0.14 \\ 
      CS~22897-008 &        4005.702 &            0.37 &            0.20 \\ 
      CS~22897-008 &        4023.377 &            0.37 &            0.30 \\ 
      CS~22898-043 &        3715.464 &            1.46 &            0.34 \\ 
      CS~22898-043 &        3951.957 &            1.50 &            0.14 \\ 
      CS~22898-043 &        4005.702 &            1.39 &            0.30 \\ 
      CS~22898-043 &        4023.377 &            1.45 &            0.11 \\ 
      CS~22898-047 &        3517.299 &            0.54 &            0.21 \\ 
      CS~22898-047 &        3545.196 &            0.51 &            0.40 \\ 
      CS~22898-047 &        3715.464 &            0.74 &            0.18 \\ 
      CS~22898-047 &        4005.702 &            0.62 &            0.20 \\ 
      CS~22937-072 &        3517.299 &            1.27 &            0.21 \\ 
      CS~22937-072 &        3545.196 &            1.39 &            0.11 \\ 
      CS~22937-072 &        3715.464 &            1.31 &            0.18 \\ 
      CS~22937-072 &        3951.957 &            1.42 &            0.14 \\ 
      CS~22937-072 &        4002.928 &            1.49 &            0.11 \\ 
      CS~22937-072 &        4005.702 &            1.43 &            0.06 \\ 
      CS~22937-072 &        4023.377 &            1.52 &            0.06 \\ 
      CS~22940-070 &        3545.196 &            2.34 &            0.30 \\ 
      CS~22940-070 &        3715.464 &            2.47 &            0.34 \\ 
      CS~22940-070 &        3951.957 &            2.57 &            0.14 \\ 
      CS~22940-070 &        4002.928 &            2.61 &            0.11 \\ 
      CS~22940-070 &        4005.702 &            2.64 &            0.11 \\ 
      CS~22940-070 &        4023.377 &            2.52 &            0.11 \\ 
      CS~22940-077 &        3517.299 &            0.93 &            0.21 \\ 
      CS~22940-077 &        3545.196 &            0.81 &            0.21 \\ 
      CS~22940-077 &        3715.464 &            0.96 &            0.18 \\ 
      CS~22940-077 &        3951.957 &            0.96 &            0.22 \\ 
      CS~22940-077 &        4005.702 &            0.93 &            0.30 \\ 
      CS~22940-077 &        4023.377 &            1.08 &            0.11 \\ 
      CS~22940-121 &        3545.196 &            0.98 &            0.30 \\ 
      CS~22940-121 &        3715.464 &            0.97 &            0.18 \\ 
      CS~22940-121 &        3951.957 &            0.88 &            0.22 \\ 
      CS~22940-121 &        4002.928 &            1.24 &            0.30 \\ 
      CS~22940-121 &        4005.702 &            1.00 &            0.11 \\ 
      CS~22940-121 &        4023.377 &            0.97 &            0.11 \\ 
      CS~22941-017 &        3517.299 &            1.02 &            0.13 \\ 
      CS~22941-017 &        3545.196 &            1.14 &            0.11 \\ 
      CS~22941-017 &        3715.464 &            1.15 &            0.33 \\ 
      CS~22941-017 &        3951.957 &            0.83 &            0.22 \\ 
      CS~22941-017 &        4005.702 &            0.88 &            0.20 \\ 
      CS~22941-017 &        4023.377 &            1.03 &            0.30 \\ 
      CS~22941-027 &        3715.464 &            1.23 &            0.25 \\ 
      CS~22941-027 &        3951.957 &            1.14 &            0.32 \\ 
      CS~22941-027 &        4005.702 &            1.39 &            0.20 \\ 
      CS~22941-027 &        4023.377 &            1.24 &            0.30 \\ 
      CS~22942-002 &        3517.299 &            0.27 &            0.09 \\ 
      CS~22942-002 &        3545.196 &            0.37 &            0.11 \\ 
      CS~22942-002 &        3715.464 &            0.64 &            0.15 \\ 
      CS~22942-002 &        3951.957 &            0.71 &            0.22 \\ 
      CS~22942-002 &        4005.702 &            0.76 &            0.20 \\ 
      CS~22942-011 &        3517.299 &            1.06 &            0.21 \\ 
      CS~22942-011 &        3545.196 &            1.18 &            0.11 \\ 
      CS~22942-011 &        3715.464 &            1.16 &            0.17 \\ 
      CS~22942-011 &        3951.957 &            1.22 &            0.22 \\ 
      CS~22942-011 &        4005.702 &            1.12 &            0.11 \\ 
      CS~22942-011 &        4023.377 &            1.12 &            0.11 \\ 
      CS~22942-035 &        3517.299 &            1.12 &            0.09 \\ 
      CS~22942-035 &        3545.196 &            0.82 &            0.07 \\ 
      CS~22942-035 &        3715.464 &            1.01 &            0.17 \\ 
      CS~22942-035 &        3951.957 &            0.68 &            0.22 \\ 
      CS~22942-035 &        4005.702 &            1.12 &            0.11 \\ 
      CS~22942-035 &        4023.377 &            1.03 &            0.11 \\ 
      CS~22943-059 &        3517.299 &            1.36 &            0.22 \\ 
      CS~22943-059 &        3545.196 &            1.59 &            0.11 \\ 
      CS~22943-059 &        3715.464 &            1.53 &            0.34 \\ 
      CS~22943-059 &        4005.702 &            1.54 &            0.11 \\ 
      CS~22943-095 &        3517.299 &            1.78 &            0.31 \\ 
      CS~22943-095 &        3545.196 &            1.83 &            0.21 \\ 
      CS~22943-095 &        3715.464 &            1.96 &            0.26 \\ 
      CS~22943-095 &        3951.957 &            1.82 &            0.22 \\ 
      CS~22943-095 &        4005.702 &            1.71 &            0.11 \\ 
      CS~22943-132 &        3517.299 &            1.11 &            0.13 \\ 
      CS~22943-132 &        3545.196 &            1.55 &            0.11 \\ 
      CS~22943-132 &        3715.464 &            1.37 &            0.18 \\ 
      CS~22943-132 &        3951.957 &            1.41 &            0.22 \\ 
      CS~22943-132 &        4005.702 &            1.56 &            0.20 \\ 
      CS~22943-132 &        4023.377 &            1.62 &            0.20 \\ 
      CS~22943-201 &        3545.196 &            1.62 &            0.30 \\ 
      CS~22943-201 &        3715.464 &            1.21 &            0.25 \\ 
      CS~22943-201 &        4023.377 &            1.40 &            0.30 \\ 
      CS~22944-014 &        3517.299 &            1.52 &            0.31 \\ 
      CS~22944-014 &        3545.196 &            1.69 &            0.21 \\ 
      CS~22944-014 &        3715.464 &            1.70 &            0.25 \\ 
      CS~22944-032 &        3517.299 &            0.98 &            0.13 \\ 
      CS~22944-032 &        3545.196 &            0.92 &            0.11 \\ 
      CS~22944-032 &        3715.464 &            0.96 &            0.15 \\ 
      CS~22944-032 &        3951.957 &            0.64 &            0.14 \\ 
      CS~22944-032 &        4005.702 &            0.90 &            0.20 \\ 
      CS~22944-032 &        4023.377 &            0.99 &            0.30 \\ 
      CS~22944-061 &        3545.196 &            1.38 &            0.21 \\ 
      CS~22945-024 &        3517.299 &            1.26 &            0.21 \\ 
      CS~22945-024 &        3545.196 &            1.39 &            0.11 \\ 
      CS~22945-024 &        3715.464 &            1.52 &            0.33 \\ 
      CS~22945-024 &        3951.957 &            1.59 &            0.22 \\ 
      CS~22945-024 &        4002.928 &            1.58 &            0.11 \\ 
      CS~22945-028 &        3517.299 &            1.30 &            0.13 \\ 
      CS~22945-028 &        3545.196 &            0.94 &            0.11 \\ 
      CS~22945-028 &        3715.464 &            0.98 &            0.17 \\ 
      CS~22945-028 &        3951.957 &            0.98 &            0.22 \\ 
      CS~22945-028 &        4005.702 &            0.88 &            0.11 \\ 
      CS~22945-028 &        4023.377 &            0.97 &            0.11 \\ 
      CS~22945-056 &        3951.957 &            1.24 &            0.22 \\ 
      CS~22945-056 &        4002.928 &            1.27 &            0.30 \\ 
      CS~22945-056 &        4005.702 &            1.12 &            0.11 \\ 
      CS~22945-056 &        4023.377 &            1.36 &            0.11 \\ 
      CS~22945-058 &        4005.702 &            1.71 &            0.11 \\ 
      CS~22945-063 &        3517.299 &            1.26 &            0.31 \\ 
      CS~22945-063 &        3545.196 &            1.49 &            0.30 \\ 
      CS~22945-063 &        3715.464 &            1.39 &            0.25 \\ 
      CS~22945-063 &        3951.957 &            1.26 &            0.22 \\ 
      CS~22945-063 &        4005.702 &            1.40 &            0.20 \\ 
      CS~22945-063 &        4023.377 &            1.49 &            0.20 \\ 
      CS~22947-187 &        3517.299 &            1.47 &            0.21 \\ 
      CS~22947-187 &        3545.196 &            1.20 &            0.30 \\ 
      CS~22947-187 &        3715.464 &            1.35 &            0.18 \\ 
      CS~22947-187 &        3951.957 &            1.53 &            0.14 \\ 
      CS~22947-187 &        4002.928 &            1.68 &            0.11 \\ 
      CS~22947-187 &        4005.702 &            1.56 &            0.11 \\ 
      CS~22947-187 &        4023.377 &            1.35 &            0.11 \\ 
      CS~22948-066 &        3517.299 &            0.90 &            0.13 \\ 
      CS~22948-066 &        3545.196 &            0.82 &            0.21 \\ 
      CS~22948-066 &        3715.464 &            1.06 &            0.17 \\ 
      CS~22948-066 &        3951.957 &            1.07 &            0.22 \\ 
      CS~22948-066 &        4005.702 &            1.02 &            0.06 \\ 
      CS~22948-066 &        4023.377 &            0.90 &            0.11 \\ 
      CS~22949-030 &        3517.299 &            1.37 &            0.31 \\ 
      CS~22949-030 &        3715.464 &            1.30 &            0.25 \\ 
      CS~22949-037 &        3517.299 &            0.38 &            0.21 \\ 
      CS~22949-037 &        3545.196 &            0.09 &            0.21 \\ 
      CS~22949-037 &        3715.464 &            0.11 &            0.24 \\ 
      CS~22949-048 &        3517.299 &            0.56 &            0.09 \\ 
      CS~22949-048 &        3545.196 &            0.52 &            0.21 \\ 
      CS~22949-048 &        3715.464 &            0.71 &            0.15 \\ 
      CS~22949-048 &        3951.957 &            0.67 &            0.10 \\ 
      CS~22949-048 &        4005.702 &            0.61 &            0.11 \\ 
      CS~22949-048 &        4023.377 &            0.40 &            0.11 \\ 
      CS~22950-046 &        3517.299 &            0.11 &            0.12 \\ 
      CS~22950-046 &        3545.196 &            0.27 &            0.11 \\ 
      CS~22950-046 &        3715.464 &            0.16 &            0.24 \\ 
      CS~22950-046 &        4005.702 &           -0.01 &            0.30 \\ 
      CS~22950-046 &        4023.377 &            0.14 &            0.30 \\ 
      CS~22951-005 &        3517.299 &            1.46 &            0.13 \\ 
      CS~22951-005 &        3545.196 &            1.56 &            0.30 \\ 
      CS~22951-005 &        3715.464 &            1.54 &            0.19 \\ 
      CS~22951-005 &        3951.957 &            1.19 &            0.22 \\ 
      CS~22951-005 &        4005.702 &            1.88 &            0.20 \\ 
      CS~22951-059 &        3517.299 &            1.33 &            0.13 \\ 
      CS~22951-059 &        3545.196 &            1.16 &            0.21 \\ 
      CS~22951-059 &        3715.464 &            1.26 &            0.25 \\ 
      CS~22951-059 &        3951.957 &            1.33 &            0.14 \\ 
      CS~22951-059 &        4005.702 &            0.93 &            0.20 \\ 
      CS~22951-077 &        3517.299 &            1.16 &            0.13 \\ 
      CS~22951-077 &        3545.196 &            1.28 &            0.21 \\ 
      CS~22951-077 &        3715.464 &            1.13 &            0.25 \\ 
      CS~22951-077 &        3951.957 &            1.40 &            0.11 \\ 
      CS~22951-077 &        4002.928 &            1.37 &            0.11 \\ 
      CS~22951-077 &        4005.702 &            1.40 &            0.11 \\ 
      CS~22951-077 &        4023.377 &            1.49 &            0.06 \\ 
      CS~22952-015 &        3517.299 &           -0.03 &            0.21 \\ 
      CS~22952-015 &        3545.196 &           -0.08 &            0.16 \\ 
      CS~22952-015 &        3715.464 &            0.20 &            0.15 \\ 
      CS~22952-015 &        3951.957 &           -0.02 &            0.10 \\ 
      CS~22952-015 &        4005.702 &            0.28 &            0.20 \\ 
      CS~22953-003 &        3517.299 &            0.78 &            0.13 \\ 
      CS~22953-003 &        3545.196 &            0.79 &            0.11 \\ 
      CS~22953-003 &        3715.464 &            0.91 &            0.17 \\ 
      CS~22953-003 &        3951.957 &            0.95 &            0.14 \\ 
      CS~22953-003 &        4005.702 &            0.87 &            0.11 \\ 
      CS~22953-003 &        4023.377 &            0.78 &            0.15 \\ 
      CS~22954-004 &        3545.196 &            1.43 &            0.11 \\ 
      CS~22954-004 &        4005.702 &            1.29 &            0.20 \\ 
      CS~22954-015 &        3517.299 &            2.19 &            0.17 \\ 
      CS~22954-015 &        3545.196 &            2.26 &            0.11 \\ 
      CS~22954-015 &        3715.464 &            2.21 &            0.19 \\ 
      CS~22954-015 &        3951.957 &            2.19 &            0.22 \\ 
      CS~22954-015 &        4005.702 &            2.16 &            0.20 \\ 
      CS~22954-015 &        4023.377 &            2.37 &            0.20 \\ 
      CS~22955-110 &        3517.299 &            2.63 &            0.10 \\ 
      CS~22955-110 &        3545.196 &            2.69 &            0.11 \\ 
      CS~22955-110 &        3715.464 &            2.47 &            0.19 \\ 
      CS~22955-110 &        3951.957 &            2.62 &            0.12 \\ 
      CS~22955-110 &        4002.928 &            2.68 &            0.06 \\ 
      CS~22955-110 &        4005.702 &            2.68 &            0.06 \\ 
      CS~22955-110 &        4023.377 &            2.68 &            0.06 \\ 
      CS~22955-174 &        3545.196 &            1.12 &            0.40 \\ 
      CS~22955-174 &        3715.464 &            1.01 &            0.18 \\ 
      CS~22955-174 &        3951.957 &            1.21 &            0.22 \\ 
      CS~22955-174 &        4005.702 &            0.95 &            0.15 \\ 
      CS~22955-174 &        4023.377 &            1.16 &            0.11 \\ 
      CS~22956-015 &        3951.957 &            1.60 &            0.32 \\ 
      CS~22956-015 &        4005.702 &            1.69 &            0.11 \\ 
      CS~22956-021 &        3517.299 &            1.64 &            0.22 \\ 
      CS~22956-021 &        3715.464 &            1.67 &            0.34 \\ 
      CS~22956-021 &        3951.957 &            1.65 &            0.41 \\ 
      CS~22956-021 &        4005.702 &            1.56 &            0.50 \\ 
      CS~22956-050 &        3517.299 &            0.68 &            0.31 \\ 
      CS~22956-050 &        3545.196 &            0.51 &            0.21 \\ 
      CS~22956-050 &        3715.464 &            0.29 &            0.24 \\ 
      CS~22956-050 &        3951.957 &            0.49 &            0.22 \\ 
      CS~22956-050 &        4005.702 &            0.34 &            0.40 \\ 
      CS~22956-050 &        4023.377 &            0.67 &            0.11 \\ 
      CS~22956-062 &        3517.299 &            1.74 &            0.31 \\ 
      CS~22956-062 &        3715.464 &            1.62 &            0.34 \\ 
      CS~22956-062 &        4005.702 &            1.54 &            0.30 \\ 
      CS~22956-102 &        4023.377 &            2.14 &            0.11 \\ 
      CS~22956-110 &        3715.464 &            1.19 &            0.25 \\ 
      CS~22956-110 &        3951.957 &            1.41 &            0.32 \\ 
      CS~22956-110 &        4005.702 &            1.47 &            0.20 \\ 
      CS~22956-114 &        3517.299 &            0.85 &            0.17 \\ 
      CS~22956-114 &        3545.196 &            0.85 &            0.11 \\ 
      CS~22956-114 &        3715.464 &            0.95 &            0.25 \\ 
      CS~22956-114 &        3951.957 &            1.04 &            0.18 \\ 
      CS~22956-114 &        4005.702 &            1.15 &            0.11 \\ 
      CS~22956-114 &        4023.377 &            1.18 &            0.11 \\ 
      CS~22957-013 &        3517.299 &            0.85 &            0.31 \\ 
      CS~22957-013 &        3545.196 &            1.20 &            0.40 \\ 
      CS~22957-013 &        3715.464 &            1.00 &            0.17 \\ 
      CS~22957-013 &        3951.957 &            1.02 &            0.14 \\ 
      CS~22957-013 &        4002.928 &            0.96 &            0.20 \\ 
      CS~22957-013 &        4005.702 &            0.93 &            0.11 \\ 
      CS~22957-013 &        4023.377 &            0.96 &            0.20 \\ 
      CS~22957-019 &        3517.299 &            2.03 &            0.22 \\ 
      CS~22957-019 &        3545.196 &            1.62 &            0.07 \\ 
      CS~22957-019 &        3715.464 &            1.73 &            0.17 \\ 
      CS~22957-019 &        3951.957 &            1.49 &            0.14 \\ 
      CS~22957-019 &        4005.702 &            1.65 &            0.06 \\ 
      CS~22957-019 &        4023.377 &            1.77 &            0.06 \\ 
      CS~22957-022 &        3545.196 &            0.80 &            0.11 \\ 
      CS~22957-022 &        3715.464 &            1.01 &            0.17 \\ 
      CS~22957-022 &        3951.957 &            0.60 &            0.14 \\ 
      CS~22957-022 &        4002.928 &            0.58 &            0.30 \\ 
      CS~22957-022 &        4005.702 &            0.88 &            0.15 \\ 
      CS~22957-022 &        4023.377 &            0.88 &            0.20 \\ 
      CS~22957-024 &        3545.196 &            1.89 &            0.11 \\ 
      CS~22957-026 &        3517.299 &            2.37 &            0.31 \\ 
      CS~22957-026 &        3545.196 &            2.23 &            0.11 \\ 
      CS~22957-026 &        3715.464 &            2.06 &            0.19 \\ 
      CS~22957-026 &        3951.957 &            2.16 &            0.14 \\ 
      CS~22957-026 &        4002.928 &            2.20 &            0.30 \\ 
      CS~22957-026 &        4005.702 &            2.14 &            0.20 \\ 
      CS~22957-026 &        4023.377 &            2.08 &            0.20 \\ 
      CS~22957-027 &        3545.196 &            1.23 &            0.11 \\ 
      CS~22957-027 &        3715.464 &            1.19 &            0.18 \\ 
      CS~22957-027 &        4002.928 &            1.07 &            0.30 \\ 
      CS~22957-036 &        3517.299 &            2.14 &            0.22 \\ 
      CS~22957-036 &        3545.196 &            2.07 &            0.21 \\ 
      CS~22957-036 &        3715.464 &            2.08 &            0.22 \\ 
      CS~22957-036 &        3951.957 &            1.97 &            0.22 \\ 
      CS~22957-036 &        4005.702 &            2.00 &            0.11 \\ 
      CS~22957-036 &        4023.377 &            2.03 &            0.11 \\ 
      CS~22958-037 &        3517.299 &            1.58 &            0.13 \\ 
      CS~22958-037 &        3545.196 &            1.78 &            0.16 \\ 
      CS~22958-037 &        3715.464 &            1.71 &            0.18 \\ 
      CS~22958-037 &        3951.957 &            1.64 &            0.14 \\ 
      CS~22958-037 &        4005.702 &            1.63 &            0.20 \\ 
      CS~22958-037 &        4023.377 &            1.42 &            0.15 \\ 
      CS~22958-052 &        3715.464 &            1.95 &            0.19 \\ 
      CS~22958-052 &        4005.702 &            1.79 &            0.30 \\ 
      CS~22958-052 &        4023.377 &            1.82 &            0.20 \\ 
      CS~22958-065 &        3517.299 &            2.03 &            0.31 \\ 
      CS~22958-065 &        3545.196 &            2.05 &            0.40 \\ 
      CS~22958-065 &        3715.464 &            1.70 &            0.25 \\ 
      CS~22958-065 &        3951.957 &            1.68 &            0.22 \\ 
      CS~22958-065 &        4005.702 &            1.86 &            0.20 \\ 
      CS~22958-074 &        3517.299 &            1.55 &            0.31 \\ 
      CS~22958-074 &        3715.464 &            1.72 &            0.25 \\ 
      CS~22958-083 &        3517.299 &            1.06 &            0.41 \\ 
      CS~22958-083 &        3545.196 &            1.03 &            0.40 \\ 
      CS~22958-083 &        3715.464 &            1.13 &            0.33 \\ 
      CS~22958-083 &        3951.957 &            0.95 &            0.11 \\ 
      CS~22958-083 &        4002.928 &            0.82 &            0.11 \\ 
      CS~22958-083 &        4005.702 &            1.00 &            0.11 \\ 
      CS~22958-083 &        4023.377 &            1.00 &            0.20 \\ 
      CS~22959-074 &        3517.299 &            1.53 &            0.13 \\ 
      CS~22959-074 &        3545.196 &            1.26 &            0.40 \\ 
      CS~22959-074 &        3715.464 &            1.48 &            0.25 \\ 
      CS~22959-074 &        3951.957 &            1.18 &            0.14 \\ 
      CS~22959-074 &        4002.928 &            1.44 &            0.11 \\ 
      CS~22959-074 &        4005.702 &            1.38 &            0.11 \\ 
      CS~22959-074 &        4023.377 &            1.35 &            0.20 \\ 
      CS~22959-139 &        4023.377 &            2.02 &            0.20 \\ 
      CS~22960-010 &        3545.196 &            1.45 &            0.11 \\ 
      CS~22960-010 &        3715.464 &            1.51 &            0.33 \\ 
      CS~22960-048 &        3517.299 &            0.48 &            0.31 \\ 
      CS~22960-048 &        3715.464 &            0.36 &            0.15 \\ 
      CS~22960-048 &        3951.957 &            0.34 &            0.14 \\ 
      CS~22960-064 &        3517.299 &            1.46 &            0.13 \\ 
      CS~22960-064 &        3545.196 &            1.22 &            0.16 \\ 
      CS~22960-064 &        3715.464 &            1.26 &            0.18 \\ 
      CS~22960-064 &        3951.957 &            1.18 &            0.14 \\ 
      CS~22960-064 &        4002.928 &            1.29 &            0.20 \\ 
      CS~22960-064 &        4005.702 &            1.23 &            0.11 \\ 
      CS~22960-064 &        4023.377 &            1.23 &            0.11 \\ 
      CS~22964-115 &        3517.299 &            1.74 &            0.13 \\ 
      CS~22964-176 &        3517.299 &            1.83 &            0.13 \\ 
      CS~22964-176 &        3715.464 &            1.68 &            0.34 \\ 
      CS~22964-176 &        3951.957 &            1.81 &            0.22 \\ 
      CS~22964-176 &        4005.702 &            1.63 &            0.20 \\ 
      CS~22964-176 &        4023.377 &            1.66 &            0.30 \\ 
      CS~22965-016 &        3715.464 &            1.04 &            0.33 \\ 
      CS~22965-016 &        3951.957 &            1.14 &            0.11 \\ 
      CS~22965-016 &        4005.702 &            1.12 &            0.06 \\ 
      CS~22965-016 &        4023.377 &            1.18 &            0.11 \\ 
      CS~22968-001 &        3951.957 &            1.47 &            0.32 \\ 
      CS~22968-014 &        3545.196 &            0.03 &            0.11 \\ 
      CS~22968-014 &        3951.957 &           -0.06 &            0.22 \\ 
      CS~22968-014 &        4005.702 &           -0.18 &            0.40 \\ 
      CS~22968-026 &        3517.299 &            1.72 &            0.10 \\ 
      CS~22968-026 &        3545.196 &            1.86 &            0.11 \\ 
      CS~22968-026 &        3715.464 &            1.83 &            0.18 \\ 
      CS~22968-026 &        4023.377 &            1.90 &            0.20 \\ 
      CS~29493-023 &        3545.196 &            1.55 &            0.30 \\ 
      CS~29493-050 &        3545.196 &            1.45 &            0.21 \\ 
      CS~29493-062 &        3517.299 &            1.45 &            0.09 \\ 
      CS~29493-062 &        3545.196 &            1.66 &            0.11 \\ 
      CS~29493-062 &        3715.464 &            1.52 &            0.18 \\ 
      CS~29493-062 &        3951.957 &            1.42 &            0.22 \\ 
      CS~29493-062 &        4005.702 &            1.52 &            0.11 \\ 
      CS~29495-005 &        3517.299 &            1.85 &            0.13 \\ 
      CS~29495-005 &        3545.196 &            1.88 &            0.11 \\ 
      CS~29495-005 &        3715.464 &            2.07 &            0.19 \\ 
      CS~29495-005 &        3951.957 &            1.93 &            0.14 \\ 
      CS~29495-005 &        4005.702 &            1.90 &            0.11 \\ 
      CS~29495-005 &        4023.377 &            2.02 &            0.11 \\ 
      CS~29495-042 &        3517.299 &            1.96 &            0.31 \\ 
      CS~29495-042 &        3545.196 &            1.48 &            0.21 \\ 
      CS~29495-042 &        3715.464 &            1.41 &            0.18 \\ 
      CS~29495-042 &        3951.957 &            1.68 &            0.22 \\ 
      CS~29495-042 &        4002.928 &            1.89 &            0.30 \\ 
      CS~29495-042 &        4005.702 &            1.89 &            0.11 \\ 
      CS~29495-042 &        4023.377 &            1.68 &            0.20 \\ 
      CS~29497-030 &        4005.702 &            2.13 &            0.40 \\ 
      CS~29498-043 &        3715.464 &            0.28 &            0.24 \\ 
      CS~29499-003 &        3517.299 &            1.81 &            0.13 \\ 
      CS~29499-003 &        3545.196 &            1.76 &            0.21 \\ 
      CS~29499-003 &        3951.957 &            1.93 &            0.22 \\ 
      CS~29499-003 &        4005.702 &            2.21 &            0.20 \\ 
      CS~29499-003 &        4023.377 &            2.00 &            0.11 \\ 
      CS~29499-058 &        3517.299 &            1.55 &            0.31 \\ 
      CS~29499-058 &        3545.196 &            1.62 &            0.21 \\ 
      CS~29499-058 &        3715.464 &            1.64 &            0.19 \\ 
      CS~29499-058 &        3951.957 &            1.73 &            0.32 \\ 
      CS~29499-060 &        3517.299 &            1.61 &            0.26 \\ 
      CS~29499-060 &        3545.196 &            1.65 &            0.11 \\ 
      CS~29502-092 &        3517.299 &            0.68 &            0.13 \\ 
      CS~29502-092 &        3545.196 &            0.60 &            0.30 \\ 
      CS~29502-092 &        3715.464 &            0.60 &            0.24 \\ 
      CS~29502-092 &        3951.957 &            0.79 &            0.14 \\ 
      CS~29502-092 &        4005.702 &            0.62 &            0.11 \\ 
      CS~29502-092 &        4023.377 &            0.89 &            0.20 \\ 
      CS~29506-007 &        4005.702 &            1.30 &            0.11 \\ 
      CS~29509-027 &        3517.299 &            1.76 &            0.31 \\ 
      CS~29509-027 &        3545.196 &            1.79 &            0.21 \\ 
      CS~29509-027 &        3715.464 &            1.73 &            0.20 \\ 
      CS~29509-027 &        3951.957 &            1.72 &            0.15 \\ 
      CS~29509-027 &        4005.702 &            1.70 &            0.11 \\ 
      CS~29509-027 &        4023.377 &            1.64 &            0.11 \\ 
      CS~29512-073 &        3517.299 &            1.80 &            0.13 \\ 
      CS~29512-073 &        3545.196 &            1.95 &            0.21 \\ 
      CS~29512-073 &        3715.464 &            1.78 &            0.16 \\ 
      CS~29512-073 &        3951.957 &            1.80 &            0.14 \\ 
      CS~29512-073 &        4002.928 &            2.09 &            0.11 \\ 
      CS~29512-073 &        4005.702 &            1.64 &            0.06 \\ 
      CS~29512-073 &        4023.377 &            1.58 &            0.11 \\ 
      CS~29513-003 &        3517.299 &            1.46 &            0.13 \\ 
      CS~29513-003 &        3545.196 &            1.58 &            0.11 \\ 
      CS~29513-003 &        3715.464 &            1.65 &            0.16 \\ 
      CS~29513-003 &        3951.957 &            1.58 &            0.11 \\ 
      CS~29513-003 &        4005.702 &            1.59 &            0.06 \\ 
      CS~29513-003 &        4023.377 &            1.56 &            0.11 \\ 
      CS~29513-014 &        3517.299 &            1.59 &            0.13 \\ 
      CS~29513-014 &        3545.196 &            1.67 &            0.50 \\ 
      CS~29513-014 &        3715.464 &            1.50 &            0.16 \\ 
      CS~29513-014 &        3951.957 &            1.61 &            0.14 \\ 
      CS~29513-014 &        4002.928 &            1.80 &            0.06 \\ 
      CS~29513-014 &        4005.702 &            1.65 &            0.06 \\ 
      CS~29513-014 &        4023.377 &            1.68 &            0.06 \\ 
      CS~29513-015 &        3545.196 &            1.42 &            0.11 \\ 
      CS~29513-032 &        3517.299 &            2.16 &            0.22 \\ 
      CS~29513-032 &        3545.196 &            2.35 &            0.11 \\ 
      CS~29513-032 &        3715.464 &            1.88 &            0.25 \\ 
      CS~29513-032 &        3951.957 &            2.04 &            0.22 \\ 
      CS~29513-032 &        4005.702 &            2.02 &            0.11 \\ 
      CS~29514-017 &        3517.299 &            1.59 &            0.21 \\ 
      CS~29514-017 &        3545.196 &            1.86 &            0.11 \\ 
      CS~29514-017 &        3715.464 &            1.61 &            0.16 \\ 
      CS~29514-017 &        3951.957 &            1.31 &            0.14 \\ 
      CS~29514-017 &        4005.702 &            1.43 &            0.11 \\ 
      CS~29514-017 &        4023.377 &            1.43 &            0.11 \\ 
      CS~29514-018 &        3517.299 &            1.60 &            0.22 \\ 
      CS~29514-018 &        3545.196 &            1.56 &            0.16 \\ 
      CS~29514-018 &        3715.464 &            1.62 &            0.19 \\ 
      CS~29514-018 &        4005.702 &            1.34 &            0.20 \\ 
      CS~29514-037 &        3545.196 &            1.35 &            0.11 \\ 
      CS~29514-037 &        3715.464 &            1.62 &            0.19 \\ 
      CS~29514-037 &        3951.957 &            1.51 &            0.14 \\ 
      CS~29514-037 &        4005.702 &            1.60 &            0.06 \\ 
      CS~29514-037 &        4023.377 &            1.63 &            0.06 \\ 
      CS~29517-018 &        3517.299 &            1.54 &            0.41 \\ 
      CS~29517-018 &        3545.196 &            1.50 &            0.21 \\ 
      CS~29517-042 &        3517.299 &            1.76 &            0.31 \\ 
      CS~29517-042 &        3545.196 &            1.59 &            0.11 \\ 
      CS~29517-042 &        3715.464 &            1.84 &            0.19 \\ 
      CS~29517-042 &        4005.702 &            1.44 &            0.30 \\ 
      CS~30312-044 &        3517.299 &            0.83 &            0.21 \\ 
      CS~30312-044 &        3715.464 &            0.65 &            0.17 \\ 
      CS~30312-044 &        3951.957 &            0.70 &            0.14 \\ 
      CS~30312-044 &        4005.702 &            0.73 &            0.20 \\ 
      CS~30312-044 &        4023.377 &            0.73 &            0.11 \\ 
      CS~30312-059 &        3517.299 &            0.82 &            0.31 \\ 
      CS~30312-059 &        3545.196 &            0.73 &            0.11 \\ 
      CS~30312-059 &        3715.464 &            0.61 &            0.24 \\ 
      CS~30312-059 &        3951.957 &            0.38 &            0.27 \\ 
      CS~30312-059 &        4005.702 &            0.60 &            0.06 \\ 
      CS~30312-059 &        4023.377 &            0.45 &            0.30 \\ 
      CS~30312-062 &        3517.299 &            1.46 &            0.13 \\ 
      CS~30312-062 &        3951.957 &            1.56 &            0.23 \\ 
      CS~30312-062 &        4005.702 &            1.41 &            0.20 \\ 
      CS~30312-100 &        3517.299 &            1.48 &            0.13 \\ 
      CS~30312-100 &        3545.196 &            1.42 &            0.07 \\ 
      CS~30312-100 &        3715.464 &            1.55 &            0.18 \\ 
      CS~30312-100 &        3951.957 &            1.38 &            0.14 \\ 
      CS~30312-100 &        4002.928 &            1.61 &            0.11 \\ 
      CS~30312-100 &        4005.702 &            1.46 &            0.06 \\ 
      CS~30312-100 &        4023.377 &            1.49 &            0.11 \\ 
      CS~30314-067 &        3517.299 &            1.37 &            0.31 \\ 
      CS~30314-067 &        3545.196 &            1.06 &            0.11 \\ 
      CS~30314-067 &        3715.464 &            0.79 &            0.17 \\ 
      CS~30314-067 &        3951.957 &            0.87 &            0.10 \\ 
      CS~30314-067 &        4002.928 &            1.01 &            0.06 \\ 
      CS~30314-067 &        4005.702 &            0.80 &            0.06 \\ 
      CS~30314-067 &        4023.377 &            0.86 &            0.11 \\ 
      CS~30339-052 &        3517.299 &            1.54 &            0.31 \\ 
      CS~30339-052 &        4005.702 &            1.64 &            0.30 \\ 
      CS~30339-052 &        4023.377 &            1.31 &            0.20 \\ 
      CS~30339-073 &        3517.299 &            0.55 &            0.31 \\ 
      CS~30492-001 &        3517.299 &            1.95 &            0.22 \\ 
      CS~30492-001 &        3545.196 &            1.94 &            0.30 \\ 
      CS~30492-001 &        3951.957 &            1.83 &            0.14 \\ 
      CS~30492-001 &        4005.702 &            1.85 &            0.11 \\ 
      CS~30492-001 &        4023.377 &            1.79 &            0.11 \\ 
      CS~30492-110 &        3517.299 &            0.85 &            0.12 \\ 
      CS~30492-110 &        3545.196 &            0.80 &            0.16 \\ 
      CS~30492-110 &        3715.464 &            0.67 &            0.24 \\ 
      CS~30492-110 &        3951.957 &            0.75 &            0.14 \\ 
      CS~30492-110 &        4005.702 &            0.63 &            0.30 \\ 
      CS~30492-110 &        4023.377 &            0.66 &            0.11 \\ 
      CS~30493-071 &        3517.299 &            1.45 &            0.31 \\ 
      CS~30493-071 &        3545.196 &            1.29 &            0.21 \\ 
      CS~30493-071 &        3715.464 &            1.43 &            0.18 \\ 
      CS~30493-071 &        3951.957 &            1.78 &            0.18 \\ 
      CS~30493-071 &        4005.702 &            1.59 &            0.06 \\ 
      CS~30494-003 &        3517.299 &            1.05 &            0.21 \\ 
      CS~30494-003 &        3545.196 &            1.02 &            0.21 \\ 
      CS~30494-003 &        3715.464 &            1.18 &            0.17 \\ 
      CS~30494-003 &        3951.957 &            1.18 &            0.18 \\ 
      CS~30494-003 &        4005.702 &            1.08 &            0.11 \\ 
      CS~30494-003 &        4023.377 &            0.87 &            0.11 \\ 
      CS~31082-001 &        3517.299 &            0.73 &            0.09 \\ 
      CS~31082-001 &        3545.196 &            0.95 &            0.21 \\ 
      CS~31082-001 &        3951.957 &            0.87 &            0.14 \\ 
      CS~31082-001 &        4002.928 &            0.81 &            0.15 \\ 
      CS~31082-001 &        4005.702 &            0.99 &            0.11 \\ 
      CS~31082-001 &        4023.377 &            0.81 &            0.15 \\ 
         G~004-036 &        3715.464 &            1.99 &            0.18 \\ 
         G~004-036 &        3951.957 &            2.03 &            0.14 \\ 
         G~004-036 &        4002.928 &            1.76 &            0.20 \\ 
         G~004-036 &        4005.702 &            2.00 &            0.15 \\ 
         G~004-036 &        4023.377 &            1.97 &            0.11 \\ 
         G~015-010 &        3517.299 &            1.58 &            0.21 \\ 
         G~015-010 &        3545.196 &            1.76 &            0.16 \\ 
         G~015-010 &        3715.464 &            1.62 &            0.18 \\ 
         G~015-010 &        4005.702 &            1.53 &            0.06 \\ 
         G~015-010 &        4023.377 &            1.50 &            0.11 \\ 
         G~025-024 &        4005.702 &            1.88 &            0.11 \\ 
         G~026-001 &        3715.464 &            2.12 &            0.18 \\ 
         G~026-001 &        3951.957 &            2.10 &            0.14 \\ 
         G~026-001 &        4002.928 &            2.16 &            0.11 \\ 
         G~026-001 &        4005.702 &            2.55 &            0.30 \\ 
         G~026-001 &        4023.377 &            2.01 &            0.30 \\ 
         G~071-055 &        3715.464 &            2.36 &            0.18 \\ 
         G~071-055 &        3951.957 &            2.06 &            0.18 \\ 
         G~071-055 &        4002.928 &            2.19 &            0.11 \\ 
         G~071-055 &        4005.702 &            2.19 &            0.06 \\ 
         G~071-055 &        4023.377 &            2.19 &            0.06 \\ 
         G~075-056 &        3951.957 &            1.96 &            0.22 \\ 
         G~075-056 &        4005.702 &            2.00 &            0.11 \\ 
         G~088-023 &        4005.702 &            2.33 &            0.30 \\ 
         G~090-003 &        3715.464 &            2.01 &            0.18 \\ 
         G~090-003 &        3951.957 &            1.64 &            0.14 \\ 
         G~090-003 &        4005.702 &            1.84 &            0.06 \\ 
         G~090-003 &        4023.377 &            1.84 &            0.06 \\ 
         G~090-025 &        3715.464 &            1.84 &            0.25 \\ 
         G~090-025 &        3951.957 &            1.90 &            0.11 \\ 
         G~090-025 &        4002.928 &            1.87 &            0.30 \\ 
         G~090-025 &        4005.702 &            1.93 &            0.11 \\ 
         G~090-025 &        4023.377 &            1.99 &            0.11 \\ 
         G~126-062 &        3715.464 &            2.34 &            0.25 \\ 
         G~126-062 &        3951.957 &            2.35 &            0.14 \\ 
         G~126-062 &        4002.928 &            2.17 &            0.30 \\ 
         G~126-062 &        4005.702 &            2.38 &            0.11 \\ 
         G~126-062 &        4023.377 &            2.32 &            0.11 \\ 
         G~137-086 &        3951.957 &            2.04 &            0.14 \\ 
         G~146-076 &        3951.957 &            1.71 &            0.18 \\ 
         G~146-076 &        4002.928 &            1.76 &            0.06 \\ 
         G~146-076 &        4005.702 &            1.82 &            0.11 \\ 
         G~146-076 &        4023.377 &            1.85 &            0.20 \\ 
         G~153-064 &        3715.464 &            3.02 &            0.34 \\ 
         G~153-064 &        3951.957 &            2.92 &            0.14 \\ 
         G~153-064 &        4002.928 &            2.91 &            0.11 \\ 
         G~153-064 &        4005.702 &            2.91 &            0.15 \\ 
         G~153-064 &        4023.377 &            3.00 &            0.11 \\ 
         G~161-073 &        3715.464 &            2.93 &            0.25 \\ 
         G~161-073 &        3951.957 &            2.65 &            0.14 \\ 
         G~161-073 &        4002.928 &            2.76 &            0.11 \\ 
         G~161-073 &        4005.702 &            2.73 &            0.11 \\ 
         G~161-073 &        4023.377 &            2.76 &            0.15 \\ 
         G~170-047 &        3715.464 &            1.23 &            0.25 \\ 
         G~170-047 &        3951.957 &            0.96 &            0.14 \\ 
         G~170-047 &        4002.928 &            1.10 &            0.15 \\ 
         G~170-047 &        4005.702 &            1.07 &            0.06 \\ 
         G~170-047 &        4023.377 &            1.01 &            0.11 \\ 
         G~180-058 &        3715.464 &            1.96 &            0.33 \\ 
         G~180-058 &        4005.702 &            1.54 &            0.40 \\ 
         G~188-022 &        3715.464 &            2.78 &            0.18 \\ 
         G~188-022 &        3951.957 &            2.55 &            0.14 \\ 
         G~188-022 &        4002.928 &            2.52 &            0.20 \\ 
         G~188-022 &        4005.702 &            2.64 &            0.11 \\ 
         G~188-022 &        4023.377 &            2.58 &            0.20 \\ 
         G~188-030 &        3715.464 &            1.96 &            0.18 \\ 
         G~188-030 &        3951.957 &            1.58 &            0.14 \\ 
         G~188-030 &        4005.702 &            1.84 &            0.20 \\ 
         G~188-030 &        4023.377 &            1.72 &            0.11 \\ 
         G~190-010 &        3715.464 &            2.07 &            0.43 \\ 
         G~190-010 &        3951.957 &            2.10 &            0.14 \\ 
         G~190-010 &        4005.702 &            2.01 &            0.20 \\ 
         G~190-010 &        4023.377 &            1.80 &            0.30 \\ 
         G~199-066 &        4023.377 &            2.03 &            0.11 \\ 
         G~201-044 &        3715.464 &            2.35 &            0.25 \\ 
         G~201-044 &        3951.957 &            2.39 &            0.18 \\ 
         G~201-044 &        4005.702 &            2.48 &            0.20 \\ 
         G~201-044 &        4023.377 &            2.36 &            0.11 \\ 
         G~234-028 &        3951.957 &            2.27 &            0.14 \\ 
         G~234-028 &        4005.702 &            2.18 &            0.11 \\ 
         G~234-028 &        4023.377 &            2.27 &            0.30 \\ 
         G~238-032 &        4005.702 &            2.72 &            0.20 \\ 
         G~238-032 &        4023.377 &            2.60 &            0.11 \\ 
         HD~106373 &        3517.299 &            1.83 &            0.22 \\ 
         HD~106373 &        3545.196 &            1.43 &            0.21 \\ 
         HD~106373 &        3715.464 &            1.62 &            0.22 \\ 
         HD~106373 &        3951.957 &            1.57 &            0.14 \\ 
         HD~106373 &        3951.957 &            1.86 &            0.14 \\ 
         HD~106373 &        4005.702 &            1.46 &            0.15 \\ 
         HD~106373 &        4005.702 &            1.54 &            0.06 \\ 
         HD~106373 &        4023.377 &            1.57 &            0.11 \\ 
         HD~106373 &        4023.377 &            1.82 &            0.20 \\ 
         HD~108317 &        3517.299 &            1.50 &            0.13 \\ 
         HD~108317 &        3545.196 &            1.47 &            0.30 \\ 
         HD~108317 &        3715.464 &            1.42 &            0.17 \\ 
         HD~108317 &        3951.957 &            1.40 &            0.14 \\ 
         HD~108317 &        3951.957 &            1.43 &            0.11 \\ 
         HD~108317 &        4002.928 &            1.42 &            0.20 \\ 
         HD~108317 &        4002.928 &            1.51 &            0.11 \\ 
         HD~108317 &        4005.702 &            1.51 &            0.06 \\ 
         HD~108317 &        4005.702 &            1.57 &            0.11 \\ 
         HD~108317 &        4023.377 &            1.42 &            0.15 \\ 
         HD~108317 &        4023.377 &            1.54 &            0.06 \\ 
          HD~11582 &        3517.299 &            2.27 &            0.21 \\ 
          HD~11582 &        3545.196 &            1.94 &            0.11 \\ 
          HD~11582 &        3715.464 &            1.86 &            0.15 \\ 
          HD~11582 &        3951.957 &            2.11 &            0.11 \\ 
          HD~11582 &        4002.928 &            2.07 &            0.11 \\ 
          HD~11582 &        4005.702 &            2.04 &            0.06 \\ 
          HD~11582 &        4023.377 &            2.04 &            0.06 \\ 
         HD~119516 &        3715.464 &            1.91 &            0.18 \\ 
         HD~119516 &        3951.957 &            1.93 &            0.11 \\ 
         HD~119516 &        4002.928 &            1.92 &            0.11 \\ 
         HD~119516 &        4005.702 &            2.01 &            0.11 \\ 
         HD~119516 &        4023.377 &            1.95 &            0.11 \\ 
         HD~122196 &        4005.702 &            2.28 &            0.11 \\ 
         HD~122196 &        4023.377 &            2.10 &            0.11 \\ 
         HD~122563 &        3545.196 &            1.16 &            0.30 \\ 
         HD~122563 &        3715.464 &            1.05 &            0.17 \\ 
         HD~122563 &        3951.957 &            0.83 &            0.18 \\ 
         HD~122563 &        3951.957 &            1.04 &            0.14 \\ 
         HD~122563 &        3951.957 &            1.04 &            0.18 \\ 
         HD~122563 &        4002.928 &            0.92 &            0.15 \\ 
         HD~122563 &        4002.928 &            1.07 &            0.06 \\ 
         HD~122563 &        4002.928 &            1.07 &            0.20 \\ 
         HD~122563 &        4005.702 &            1.01 &            0.11 \\ 
         HD~122563 &        4005.702 &            1.07 &            0.06 \\ 
         HD~122563 &        4005.702 &            1.07 &            0.15 \\ 
         HD~122563 &        4023.377 &            1.07 &            0.15 \\ 
         HD~122563 &        4023.377 &            1.10 &            0.06 \\ 
         HD~122563 &        4023.377 &            1.13 &            0.11 \\ 
         HD~126238 &        3517.299 &            1.90 &            0.31 \\ 
         HD~126238 &        3545.196 &            2.00 &            0.21 \\ 
         HD~126238 &        3715.464 &            1.84 &            0.21 \\ 
         HD~126238 &        3951.957 &            1.85 &            0.10 \\ 
         HD~126238 &        4002.928 &            1.80 &            0.06 \\ 
         HD~126238 &        4005.702 &            1.86 &            0.11 \\ 
         HD~126238 &        4023.377 &            1.89 &            0.11 \\ 
         HD~126587 &        3517.299 &            0.78 &            0.09 \\ 
         HD~126587 &        3545.196 &            0.70 &            0.07 \\ 
         HD~126587 &        3715.464 &            0.72 &            0.15 \\ 
         HD~126587 &        3951.957 &            0.83 &            0.10 \\ 
         HD~126587 &        4002.928 &            0.74 &            0.11 \\ 
         HD~126587 &        4005.702 &            0.80 &            0.06 \\ 
         HD~126587 &        4023.377 &            0.77 &            0.06 \\ 
         HD~128279 &        3517.299 &            1.54 &            0.09 \\ 
         HD~128279 &        3545.196 &            1.45 &            0.07 \\ 
         HD~128279 &        3715.464 &            1.46 &            0.15 \\ 
         HD~128279 &        3951.957 &            1.44 &            0.11 \\ 
         HD~128279 &        4002.928 &            1.52 &            0.11 \\ 
         HD~128279 &        4005.702 &            1.52 &            0.06 \\ 
         HD~128279 &        4023.377 &            1.46 &            0.06 \\ 
         HD~132475 &        3517.299 &            2.61 &            0.13 \\ 
         HD~132475 &        3545.196 &            2.48 &            0.11 \\ 
         HD~132475 &        3715.464 &            1.92 &            0.18 \\ 
         HD~132475 &        3715.464 &            2.52 &            0.18 \\ 
         HD~132475 &        3951.957 &            2.48 &            0.11 \\ 
         HD~132475 &        3951.957 &            2.51 &            0.14 \\ 
         HD~132475 &        4002.928 &            2.34 &            0.11 \\ 
         HD~132475 &        4002.928 &            2.40 &            0.30 \\ 
         HD~132475 &        4005.702 &            2.37 &            0.11 \\ 
         HD~132475 &        4005.702 &            2.43 &            0.06 \\ 
         HD~132475 &        4023.377 &            2.37 &            0.06 \\ 
         HD~132475 &        4023.377 &            2.46 &            0.11 \\ 
          HD~13979 &        3517.299 &            1.29 &            0.09 \\ 
          HD~13979 &        3545.196 &            1.21 &            0.07 \\ 
          HD~13979 &        3715.464 &            1.30 &            0.15 \\ 
          HD~13979 &        3951.957 &            1.16 &            0.11 \\ 
          HD~13979 &        4002.928 &            1.06 &            0.06 \\ 
          HD~13979 &        4005.702 &            1.14 &            0.06 \\ 
          HD~13979 &        4023.377 &            1.36 &            0.06 \\ 
          HD~16031 &        3715.464 &            2.63 &            0.34 \\ 
          HD~16031 &        3951.957 &            1.98 &            0.14 \\ 
          HD~16031 &        4002.928 &            1.83 &            0.30 \\ 
          HD~16031 &        4005.702 &            2.22 &            0.06 \\ 
          HD~16031 &        4023.377 &            2.16 &            0.11 \\ 
         HD~175305 &        3715.464 &            2.19 &            0.25 \\ 
         HD~175305 &        3951.957 &            2.34 &            0.14 \\ 
         HD~175305 &        4002.928 &            2.30 &            0.11 \\ 
         HD~175305 &        4005.702 &            2.33 &            0.20 \\ 
         HD~175305 &        4023.377 &            2.42 &            0.11 \\ 
         HD~175606 &        3517.299 &            1.99 &            0.31 \\ 
         HD~175606 &        3545.196 &            1.83 &            0.21 \\ 
         HD~175606 &        3715.464 &            1.89 &            0.18 \\ 
         HD~175606 &        3951.957 &            1.81 &            0.14 \\ 
         HD~175606 &        4005.702 &            1.84 &            0.11 \\ 
         HD~175606 &        4023.377 &            1.84 &            0.20 \\ 
         HD~178443 &        3517.299 &            2.41 &            0.31 \\ 
         HD~178443 &        3545.196 &            2.38 &            0.30 \\ 
         HD~178443 &        3715.464 &            1.95 &            0.21 \\ 
         HD~178443 &        3951.957 &            2.04 &            0.14 \\ 
         HD~178443 &        4002.928 &            2.01 &            0.11 \\ 
         HD~178443 &        4005.702 &            2.04 &            0.06 \\ 
         HD~178443 &        4023.377 &            1.95 &            0.06 \\ 
         HD~184266 &        3715.464 &            2.20 &            0.25 \\ 
         HD~184266 &        3951.957 &            2.25 &            0.14 \\ 
         HD~184266 &        4002.928 &            2.27 &            0.11 \\ 
         HD~184266 &        4005.702 &            2.24 &            0.20 \\ 
         HD~184266 &        4023.377 &            2.24 &            0.25 \\ 
         HD~186478 &        3517.299 &            1.44 &            0.51 \\ 
         HD~186478 &        3545.196 &            1.18 &            0.30 \\ 
         HD~186478 &        3715.464 &            1.07 &            0.17 \\ 
         HD~186478 &        3951.957 &            1.21 &            0.18 \\ 
         HD~186478 &        4002.928 &            1.18 &            0.11 \\ 
         HD~186478 &        4005.702 &            1.24 &            0.11 \\ 
         HD~186478 &        4023.377 &            1.18 &            0.06 \\ 
         HD~188510 &        3715.464 &            2.26 &            0.18 \\ 
         HD~188510 &        3951.957 &            2.14 &            0.14 \\ 
         HD~188510 &        4002.928 &            2.08 &            0.11 \\ 
         HD~188510 &        4005.702 &            2.20 &            0.11 \\ 
         HD~188510 &        4023.377 &            2.14 &            0.11 \\ 
         HD~193901 &        3517.299 &            2.76 &            0.13 \\ 
         HD~193901 &        3545.196 &            2.66 &            0.21 \\ 
         HD~193901 &        3715.464 &            2.70 &            0.18 \\ 
         HD~193901 &        3951.957 &            2.64 &            0.14 \\ 
         HD~193901 &        4002.928 &            2.53 &            0.11 \\ 
         HD~193901 &        4005.702 &            2.62 &            0.06 \\ 
         HD~193901 &        4023.377 &            2.86 &            0.11 \\ 
          HD~19445 &        3715.464 &            1.63 &            0.18 \\ 
          HD~19445 &        3951.957 &            1.55 &            0.11 \\ 
          HD~19445 &        4005.702 &            1.73 &            0.20 \\ 
          HD~19445 &        4023.377 &            1.67 &            0.20 \\ 
         HD~196892 &        3715.464 &            2.88 &            0.43 \\ 
         HD~196892 &        3951.957 &            2.84 &            0.14 \\ 
         HD~196892 &        4002.928 &            2.83 &            0.20 \\ 
         HD~196892 &        4005.702 &            2.89 &            0.11 \\ 
         HD~196892 &        4023.377 &            2.89 &            0.11 \\ 
         HD~196944 &        3517.299 &            1.49 &            0.13 \\ 
         HD~196944 &        3545.196 &            1.49 &            0.11 \\ 
         HD~196944 &        3715.464 &            1.34 &            0.18 \\ 
         HD~196944 &        3951.957 &            1.61 &            0.11 \\ 
         HD~196944 &        4002.928 &            1.58 &            0.20 \\ 
         HD~196944 &        4005.702 &            1.58 &            0.11 \\ 
         HD~196944 &        4023.377 &            1.49 &            0.15 \\ 
         HD~200654 &        3517.299 &            1.05 &            0.09 \\ 
         HD~200654 &        3545.196 &            0.99 &            0.07 \\ 
         HD~200654 &        3715.464 &            1.10 &            0.15 \\ 
         HD~200654 &        3951.957 &            0.86 &            0.14 \\ 
         HD~200654 &        4002.928 &            0.82 &            0.11 \\ 
         HD~200654 &        4005.702 &            0.97 &            0.11 \\ 
         HD~200654 &        4023.377 &            1.03 &            0.11 \\ 
         HD~201891 &        3715.464 &            2.88 &            0.18 \\ 
         HD~201891 &        3951.957 &            2.80 &            0.11 \\ 
         HD~201891 &        4002.928 &            2.80 &            0.11 \\ 
         HD~201891 &        4005.702 &            2.86 &            0.11 \\ 
         HD~201891 &        4023.377 &            2.89 &            0.11 \\ 
         HD~214362 &        3951.957 &            1.89 &            0.14 \\ 
         HD~214362 &        4002.928 &            1.91 &            0.11 \\ 
         HD~214362 &        4005.702 &            2.06 &            0.11 \\ 
         HD~214362 &        4023.377 &            1.88 &            0.20 \\ 
          HD~21581 &        3517.299 &            2.61 &            0.31 \\ 
          HD~21581 &        3715.464 &            2.14 &            0.25 \\ 
          HD~21581 &        3951.957 &            2.17 &            0.14 \\ 
          HD~21581 &        4002.928 &            2.31 &            0.20 \\ 
          HD~21581 &        4005.702 &            2.28 &            0.06 \\ 
          HD~21581 &        4023.377 &            2.34 &            0.06 \\ 
         HD~219617 &        3715.464 &            2.24 &            0.21 \\ 
         HD~219617 &        3951.957 &            2.20 &            0.14 \\ 
         HD~219617 &        4002.928 &            2.40 &            0.15 \\ 
         HD~219617 &        4005.702 &            2.28 &            0.11 \\ 
         HD~219617 &        4023.377 &            2.13 &            0.11 \\ 
         HD~220127 &        3517.299 &            2.53 &            0.21 \\ 
         HD~220127 &        3545.196 &            2.35 &            0.21 \\ 
         HD~220127 &        3715.464 &            2.12 &            0.18 \\ 
         HD~220127 &        3951.957 &            2.31 &            0.14 \\ 
         HD~220127 &        4002.928 &            2.22 &            0.06 \\ 
         HD~220127 &        4005.702 &            2.24 &            0.11 \\ 
         HD~220127 &        4023.377 &            2.25 &            0.11 \\ 
         HD~237846 &        3715.464 &            0.86 &            0.33 \\ 
         HD~237846 &        3951.957 &            0.63 &            0.22 \\ 
         HD~237846 &        4005.702 &            0.58 &            0.20 \\ 
         HD~237846 &        4023.377 &            0.43 &            0.40 \\ 
          HD~26169 &        3517.299 &            1.19 &            0.12 \\ 
          HD~26169 &        3545.196 &            1.38 &            0.30 \\ 
          HD~26169 &        3715.464 &            1.10 &            0.21 \\ 
          HD~26169 &        3951.957 &            1.11 &            0.10 \\ 
          HD~26169 &        4002.928 &            1.27 &            0.06 \\ 
          HD~26169 &        4005.702 &            1.18 &            0.11 \\ 
          HD~26169 &        4023.377 &            1.21 &            0.11 \\ 
          HD~26297 &        3517.299 &            2.61 &            0.21 \\ 
          HD~26297 &        3545.196 &            2.35 &            0.21 \\ 
          HD~26297 &        3715.464 &            1.88 &            0.24 \\ 
          HD~26297 &        3951.957 &            2.23 &            0.13 \\ 
          HD~26297 &        4002.928 &            2.13 &            0.20 \\ 
          HD~26297 &        4005.702 &            2.19 &            0.06 \\ 
          HD~26297 &        4023.377 &            2.19 &            0.11 \\ 
          HD~31128 &        3715.464 &            2.11 &            0.18 \\ 
          HD~31128 &        3951.957 &            2.04 &            0.14 \\ 
          HD~31128 &        4002.928 &            1.94 &            0.11 \\ 
          HD~31128 &        4005.702 &            2.15 &            0.11 \\ 
          HD~31128 &        4023.377 &            2.03 &            0.11 \\ 
          HD~45282 &        3715.464 &            2.18 &            0.18 \\ 
          HD~45282 &        3951.957 &            2.30 &            0.14 \\ 
          HD~45282 &        4002.928 &            2.33 &            0.11 \\ 
          HD~45282 &        4005.702 &            2.36 &            0.11 \\ 
          HD~45282 &        4023.377 &            2.33 &            0.06 \\ 
           HD~6268 &        3517.299 &            1.36 &            0.31 \\ 
           HD~6268 &        3545.196 &            1.49 &            0.30 \\ 
           HD~6268 &        3715.464 &            1.08 &            0.17 \\ 
           HD~6268 &        3951.957 &            1.43 &            0.14 \\ 
           HD~6268 &        4002.928 &            1.25 &            0.11 \\ 
           HD~6268 &        4005.702 &            1.19 &            0.11 \\ 
           HD~6268 &        4023.377 &            1.22 &            0.11 \\ 
          HD~88609 &        3951.957 &            0.79 &            0.10 \\ 
          HD~88609 &        4002.928 &            0.75 &            0.11 \\ 
          HD~88609 &        4005.702 &            0.75 &            0.11 \\ 
          HD~88609 &        4023.377 &            0.90 &            0.20 \\ 
          HD~94028 &        3715.464 &            1.98 &            0.18 \\ 
          HD~94028 &        3951.957 &            2.36 &            0.22 \\ 
          HD~94028 &        4002.928 &            2.14 &            0.20 \\ 
          HD~94028 &        4005.702 &            2.29 &            0.20 \\ 
          HD~94028 &        4023.377 &            2.35 &            0.11 \\ 
      HE~0454$-$4758 &        3715.464 &            0.67 &            0.25 \\ 
      HE~0454$-$4758 &        3951.957 &            0.94 &            0.14 \\ 
      HE~0454$-$4758 &        4023.377 &            0.79 &            0.20 \\ 
      HE~1124$-$2335 &        3545.196 &            0.67 &            0.26 \\ 
      HE~1124$-$2335 &        3715.464 &            0.79 &            0.25 \\ 
      HE~1124$-$2335 &        3951.957 &            0.62 &            0.14 \\ 
      HE~1124$-$2335 &        4005.702 &            0.84 &            0.11 \\ 
      HE~1320$-$1339 &        3517.299 &            1.15 &            0.21 \\ 
      HE~1320$-$1339 &        3545.196 &            1.08 &            0.11 \\ 
      HE~1320$-$1339 &        3715.464 &            1.13 &            0.20 \\ 
      HE~1320$-$1339 &        3951.957 &            0.84 &            0.22 \\ 
      HE~1320$-$1339 &        3951.957 &            1.17 &            0.14 \\ 
      HE~1320$-$1339 &        4002.928 &            1.12 &            0.11 \\ 
      HE~1320$-$1339 &        4005.702 &            1.03 &            0.11 \\ 
      HE~1320$-$1339 &        4005.702 &            1.09 &            0.11 \\ 
      HE~1320$-$1339 &        4023.377 &            1.09 &            0.11 \\ 
      HE~1320$-$1339 &        4023.377 &            1.09 &            0.11 \\ 
         HIP~99423 &        3715.464 &            2.60 &            0.21 \\ 
         HIP~99423 &        3951.957 &            2.62 &            0.14 \\ 
         HIP~99423 &        4002.928 &            2.54 &            0.20 \\ 
         HIP~99423 &        4005.702 &            2.57 &            0.06 \\ 
         HIP~99423 &        4023.377 &            2.63 &            0.06 \\ 
\enddata      
\tablecomments{%
The model atmosphere uncertainty is not included in here for reasons 
discussed in Section~\ref{uncertainties}
}
\end{deluxetable}

==> tab04.tex <==
\startlongtable
\begin{deluxetable*}{ccccccccccccccccc}
\tablecaption{Final Abundances for the Sample
\label{vtab}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablehead{
\multicolumn{6}{c}{} &
\multicolumn{5}{c}{V~\textsc{i}} &
\colhead{ } &
\multicolumn{5}{c}{V~\textsc{ii}} \\
\cline{7-11}
\cline{13-17}
\colhead{Star} &
\colhead{Class} &
\colhead{\teff (K)} &
\colhead{\logg} &
\colhead{[Fe~\textsc{i}/H]} &
\colhead{[Fe~\textsc{ii}/H]} &
\colhead{U. L.}\tablenotemark{a} &
\colhead{U. L. $\lambda$} &
\colhead{[V~\textsc{i}/Fe~\textsc{i}]} &
\colhead{$\sigma$} &
\colhead{$N$} &
\colhead{ } &
\colhead{U. L.}\tablenotemark{a} &
\colhead{U. L. $\lambda$} &
\colhead{[V~\textsc{ii}/Fe~\textsc{ii}]} &
\colhead{$\sigma$} &
\colhead{$N$}
}
\startdata
BD~$+$10\degree2495 &    RG &       4890 &       1.85 &      -2.16 &      -2.14 &          0 &         -- &      -0.36 &        0.10 &          4 &            &          0 &         -- &      -0.01 &       0.19 &          5 \\ 
BD~$+$19\degree1185a &    MS &       5440 &       4.30 &      -1.25 &      -1.25 &          0 &         -- &      -0.21 &       0.12 &          4 &            &          0 &         -- &       0.15 &       0.14 &          4 \\ 
BD~$+$24\degree1676 &    SG &       6140 &       3.75 &      -2.70 &      -2.54 &          1 &   4111.779 &       0.81 &         -- &          0 &            &          0 &         -- &       0.32 &       0.23 &          3 \\ 
BD~$+$26\degree3578 &    SG &       6060 &       3.75 &      -2.60 &      -2.41 &          0 &         -- &       0.10 &       0.14 &          1 &            &          0 &         -- &       0.22 &       0.22 &          2 \\ 
BD~$+$29\degree2356 &    RG &       4710 &       1.75 &      -1.73 &      -1.62 &          0 &         -- &      -0.24 &        0.20 &          1 &            &          0 &         -- &       0.16 &       0.18 &          4 \\ 
BD~$+$44\degree0493 &    RG &       5040 &       2.10 &      -4.28 &      -4.26 &          1 &   4111.779 &       1.27 &         -- &          0 &            &          1 &   3715.464 &       0.97 &         -- &          0 \\ 
BD~$+$80\degree0245 &    RG &       5360 &       3.15 &      -2.04 &      -2.01 &          0 &         -- &      -0.61 &       0.14 &          1 &            &          0 &         -- &      -0.39 &       0.19 &          3 \\ 
BD~$-$01\degree2582 &    RG &       4920 &       1.80 &      -2.62 &      -2.65 &          0 &         -- &      -0.30 &       0.13 &          1 &            &          0 &         -- &       0.02 &       0.18 &          5 \\ 
BD~$-$15\degree5781 &    RG &       4550 &       0.70 &      -2.92 &      -2.87 &          0 &         -- &      -0.22 &       0.12 &          4 &            &          0 &         -- &      -0.06 &       0.18 &          7 \\ 
BD~$-$18\degree5550 &    RG &       4660 &       1.05 &      -3.20 &      -3.15 &          0 &         -- &      -0.08 &        0.10 &          1 &            &          0 &         -- &       0.05 &        0.20 &          5 \\ 
BD~$-$20\degree6008 &    RG &       4540 &       0.65 &      -3.00 &      -3.05 &          0 &         -- &      -0.28 &       0.12 &          4 &            &          0 &         -- &       0.05 &       0.22 &          7 \\ 
CD~$-$24\degree1782 &    RG &       4950 &       1.90 &      -3.05 &      -3.02 &          0 &         -- &      -0.08 &       0.13 &          3 &            &          0 &         -- &       0.15 &       0.21 &          6 \\ 
CD~$-$30\degree0298 &    RG &       4810 &       1.50 &      -3.77 &      -3.72 &          1 &    4379.23 &       0.25 &         -- &          0 &            &          0 &         -- &       0.01 &       0.22 &          4 \\ 
CD~$-$36\degree1052 &    HB &       6030 &       2.05 &      -1.87 &      -1.86 &          0 &         -- &       0.04 &       0.14 &          4 &            &          0 &         -- &       0.06 &       0.21 &          7 \\ 
CD~$-$38\degree0245 &    RG &       4520 &       0.65 &      -4.59 &      -4.50 &          1 &    4379.23 &       0.98 &         -- &          0 &            &          1 &   3517.299 &       0.55 &         -- &          0 \\ 
   CS~22166-016 &    RG &       4900 &       1.75 &      -3.22 &      -3.09 &          0 &         -- &      -0.06 &       0.13 &          3 &            &          0 &         -- &       0.12 &       0.19 &          7 \\ 
   CS~22169-008 &    SG &       5810 &       3.60 &      -2.85 &      -2.59 &          0 &         -- &       0.38 &       0.14 &          1 &            &          0 &         -- &       0.18 &       0.22 &          5 \\ 
   CS~22169-035 &    RG &       4480 &       0.50 &      -3.31 &      -3.12 &          0 &         -- &      -0.55 &       0.15 &          4 &            &          0 &         -- &      -0.50 &       0.25 &          5 \\ 
   CS~22171-031 &    SG &       6010 &       3.70 &      -2.54 &      -2.42 &          0 &         -- &       0.12 &       0.31 &          1 &            &          0 &         -- &       0.36 &       0.24 &          6 \\ 
   CS~22171-037 &    SG &       6110 &       3.65 &      -3.63 &      -3.35 &          1 &    4379.23 &       1.65 &         -- &          0 &            &          1 &   3715.464 &       1.32 &         -- &          0 \\ 
   CS~22172-029 &    RG &       4960 &       1.90 &      -2.68 &      -2.70 &          0 &         -- &      -0.15 &       0.09 &          4 &            &          0 &         -- &       0.12 &       0.22 &          7 \\ 
   CS~22174-020 &    SG &       5840 &       3.55 &      -3.29 &      -3.02 &          1 &    4379.23 &       1.19 &         -- &          0 &            &          0 &         -- &       0.65 &       0.38 &          1 \\ 
   CS~22177-009 &    SG &       5940 &       3.55 &      -3.42 &      -3.37 &          1 &   4408.196 &       1.04 &         -- &          0 &            &          0 &         -- &       0.69 &       0.37 &          1 \\ 
   CS~22177-010 &    SG &       6050 &       3.70 &      -3.00 &      -2.88 &          1 &   4111.779 &       1.02 &         -- &          0 &            &          0 &         -- &       0.23 &       0.31 &          1 \\ 
   CS~22180-014 &    SG &       5780 &       3.55 &      -2.86 &      -2.90 &          0 &         -- &       0.30 &       0.11 &          2 &            &          0 &         -- &       0.23 &       0.25 &          2 \\ 
   CS~22182-033 &    SG &       5810 &       3.60 &      -2.65 &      -2.47 &          0 &         -- &       0.13 &       0.14 &          1 &            &          0 &         -- &       0.20 &       0.22 &          4 \\ 
   CS~22182-047 &    SG &       5640 &       3.60 &      -2.18 &      -1.99 &          0 &         -- &       0.04 &        0.10 &          2 &            &          0 &         -- &       0.05 &       0.22 &          7 \\ 
   CS~22183-031 &    RG &       4850 &       1.60 &      -3.57 &      -3.50 &          0 &         -- &       0.12 &        0.10 &          3 &            &          0 &         -- &       0.26 &       0.18 &          5 \\ 
   CS~22185-007 &    RG &       4730 &       1.30 &      -3.06 &      -3.02 &          0 &         -- &      -0.04 &        0.10 &          3 &            &          0 &         -- &       0.17 &        0.20 &          7 \\ 
   CS~22186-002 &    SG &       5500 &       3.35 &      -2.72 &      -2.50 &          0 &         -- &      -0.01 &       0.13 &          1 &            &          0 &         -- &      -0.01 &       0.24 &          6 \\ 
   CS~22186-017 &    SG &       5770 &       3.55 &      -2.82 &      -2.90 &          0 &         -- &       0.37 &        0.20 &          2 &            &          0 &         -- &       0.41 &       0.22 &          2 \\ 
   CS~22186-023 &    RG &       4820 &       1.55 &      -3.04 &      -2.89 &          0 &         -- &      -0.25 &       0.09 &          2 &            &          0 &         -- &       0.03 &        0.20 &          7 \\ 
   CS~22189-009 &    RG &       4540 &       0.60 &      -3.92 &      -3.85 &          0 &         -- &      -0.20 &        0.10 &          2 &            &          0 &         -- &      -0.06 &       0.22 &          6 \\ 
   CS~22191-029 &    HB &       5810 &       1.55 &      -2.94 &      -2.94 &          1 &   4111.779 &       0.66 &         -- &          0 &            &          0 &         -- &       0.16 &       0.21 &          4 \\ 
   CS~22871-104 &    SG &       6370 &       4.00 &      -2.20 &      -2.06 &          1 &   4389.979 &       0.75 &         -- &          0 &            &          1 &   4005.702 &       0.61 &         -- &          0 \\ 
   CS~22872-102 &    SG &       6020 &       3.65 &      -2.85 &      -2.82 &          1 &   4111.779 &       0.83 &         -- &          0 &            &          1 &   4005.702 &       0.65 &         -- &          0 \\ 
   CS~22873-072 &    SG &       6030 &       3.70 &      -3.08 &      -2.86 &          1 &   4111.779 &       1.11 &         -- &          0 &            &          1 &   3951.957 &       0.35 &         -- &          0 \\ 
   CS~22873-128 &    RG &       4710 &       1.20 &      -3.32 &      -3.24 &          0 &         -- &       0.00 &       0.09 &          3 &            &          0 &         -- &       0.19 &        0.20 &          6 \\ 
   CS~22874-123 &    SG &       6240 &       3.80 &      -2.79 &      -2.61 &          1 &    4379.23 &       1.29 &         -- &          0 &            &          1 &   3951.957 &       0.56 &         -- &          0 \\ 
   CS~22875-029 &    HB &       5990 &       1.85 &      -2.71 &      -2.69 &          1 &    4379.23 &       0.75 &         -- &          0 &            &          0 &         -- &       0.24 &        0.20 &          5 \\ 
   CS~22876-040 &    SG &       6090 &       3.80 &      -2.47 &      -2.21 &          0 &         -- &       0.57 &       0.14 &          1 &            &          0 &         -- &       0.17 &       0.22 &          4 \\ 
   CS~22877-001 &    RG &       4790 &       1.45 &      -3.31 &      -3.24 &          0 &         -- &      -0.42 &        0.10 &          1 &            &          0 &         -- &      -0.13 &        0.20 &          6 \\ 
   CS~22877-011 &    RG &       4950 &       1.90 &      -3.23 &      -3.12 &          0 &         -- &       0.02 &       0.09 &          3 &            &          0 &         -- &       0.06 &       0.19 &          6 \\ 
   CS~22877-015 &    SG &       6150 &       3.85 &      -2.12 &      -2.00 &          0 &         -- &      -0.03 &       0.31 &          1 &            &          0 &         -- &       0.27 &       0.22 &          3 \\ 
   CS~22877-051 &    SG &       6050 &       3.70 &      -3.03 &      -2.77 &          1 &   4111.779 &       1.01 &         -- &          0 &            &          1 &   3545.196 &       0.58 &         -- &          0 \\ 
   CS~22878-002 &    SG &       5850 &       3.55 &      -2.97 &      -3.10 &          1 &   4111.779 &       0.63 &         -- &          0 &            &          1 &   3951.957 &       0.82 &         -- &          0 \\ 
   CS~22878-027 &    SG &       5820 &       3.55 &      -2.92 &      -2.97 &          1 &   4111.779 &       0.88 &         -- &          0 &            &          1 &   4005.702 &       0.78 &         -- &          0 \\ 
   CS~22878-101 &    RG &       4650 &       1.05 &      -3.53 &      -3.30 &          0 &         -- &      -0.04 &        0.10 &          1 &            &          0 &         -- &       0.02 &       0.21 &          7 \\ 
   CS~22879-012 &    SG &       6020 &       3.65 &      -3.01 &      -2.81 &          1 &    4379.23 &       1.02 &         -- &          0 &            &          1 &   4005.702 &       0.52 &         -- &          0 \\ 
   CS~22879-029 &    SG &       5920 &       3.70 &      -2.55 &      -2.35 &          0 &         -- &       0.22 &       0.22 &          1 &            &          0 &         -- &       0.19 &       0.24 &          5 \\ 
   CS~22879-051 &    SG &       6190 &       3.75 &      -3.02 &      -2.85 &          1 &   4111.779 &       1.46 &         -- &          0 &            &          1 &   3517.299 &       0.85 &         -- &          0 \\ 
   CS~22879-094 &    SG &       5820 &       3.60 &      -3.15 &      -2.81 &          1 &    4379.23 &       0.79 &         -- &          0 &            &          1 &   3517.299 &       0.63 &         -- &          0 \\ 
   CS~22879-097 &    HB &       5640 &       1.55 &      -2.66 &      -2.64 &          0 &         -- &       0.55 &       0.31 &          1 &            &          0 &         -- &       0.17 &       0.21 &          7 \\ 
   CS~22879-103 &    HB &       5720 &       1.60 &      -2.16 &      -2.15 &          0 &         -- &      -0.11 &       0.18 &          4 &            &          0 &         -- &       0.11 &        0.20 &          7 \\ 
   CS~22880-067 &    SG &       5570 &       3.35 &      -3.23 &      -3.37 &          1 &   4389.979 &       0.75 &         -- &          0 &            &          1 &   3715.464 &       1.00 &         -- &          0 \\ 
   CS~22880-086 &    RG &       4960 &       1.90 &      -3.28 &      -3.25 &          0 &         -- &      -0.06 &        0.10 &          2 &            &          0 &         -- &       0.14 &       0.21 &          6 \\ 
   CS~22881-032 &    SG &       5430 &       3.20 &      -3.55 &      -3.10 &          1 &   4408.196 &       1.03 &         -- &          0 &            &          1 &   3715.464 &       0.70 &         -- &          0 \\ 
   CS~22881-036 &    SG &       5940 &       3.70 &      -2.34 &      -2.37 &          0 &         -- &       0.18 &       0.22 &          1 &            &          0 &         -- &       0.27 &       0.28 &          5 \\ 
   CS~22881-039 &    HB &       6170 &       2.05 &      -2.79 &      -2.79 &          1 &   4111.779 &       1.08 &         -- &          0 &            &          0 &         -- &       0.20 &       0.21 &          2 \\ 
   CS~22881-070 &    SG &       6020 &       3.70 &      -2.96 &      -2.73 &          1 &   4111.779 &       0.95 &         -- &          0 &            &          0 &         -- &       0.41 &       0.27 &          4 \\ 
   CS~22882-001 &    HB &       5930 &       1.90 &      -2.62 &      -2.62 &          0 &         -- &       0.66 &       0.26 &          1 &            &          0 &         -- &       0.24 &       0.22 &          7 \\ 
   CS~22882-006 &    SG &       5800 &       3.60 &      -2.94 &      -2.66 &          0 &         -- &       0.38 &       0.22 &          1 &            &          0 &         -- &       0.31 &       0.26 &          5 \\ 
   CS~22882-012 &    SG &       6290 &       3.80 &      -2.76 &      -2.75 &          1 &   4111.779 &       1.14 &         -- &          0 &            &          1 &   4005.702 &       0.53 &         -- &          0 \\ 
   CS~22882-030 &    SG &       5580 &       3.40 &      -3.47 &      -3.14 &          1 &    4379.23 &       0.84 &         -- &          0 &            &          1 &   3715.464 &       0.77 &         -- &          0 \\ 
   CS~22883-037 &    HB &       5800 &       1.50 &      -2.01 &      -1.97 &          0 &         -- &      -0.07 &       0.11 &          3 &            &          0 &         -- &       0.04 &       0.21 &          6 \\ 
   CS~22884-020 &    SG &       6040 &       3.75 &      -2.48 &      -2.27 &          0 &         -- &       0.21 &        0.10 &          2 &            &          0 &         -- &       0.42 &       0.23 &          3 \\ 
   CS~22884-108 &    SG &       6320 &       3.75 &      -3.10 &      -3.21 &          1 &   4111.779 &       1.48 &         -- &          0 &            &          1 &   4005.702 &       0.99 &         -- &          0 \\ 
   CS~22885-040 &    SG &       6160 &       3.75 &      -2.78 &      -2.60 &          1 &    4379.23 &       0.74 &         -- &          0 &            &          0 &         -- &       0.27 &       0.26 &          3 \\ 
   CS~22885-096 &    RG &       4580 &       0.75 &      -4.41 &      -4.21 &          1 &    4379.23 &       0.53 &         -- &          0 &            &          0 &         -- &       0.17 &        0.20 &          3 \\ 
   CS~22885-203 &    SG &       5820 &       3.60 &      -2.73 &      -2.57 &          1 &   4111.779 &       0.68 &         -- &          0 &            &          1 &   3517.299 &       0.12 &         -- &          0 \\ 
   CS~22886-003 &    SG &       5970 &       3.65 &      -2.92 &      -2.87 &          1 &    4379.23 &       0.79 &         -- &          0 &            &          0 &         -- &       0.64 &       0.22 &          2 \\ 
   CS~22886-012 &    SG &       5650 &       3.50 &      -2.88 &      -2.61 &          0 &         -- &       0.43 &       0.22 &          1 &            &          0 &         -- &       0.46 &       0.28 &          5 \\ 
   CS~22886-013 &    HB &       6200 &       1.75 &      -2.58 &      -2.60 &          1 &   4111.779 &       0.77 &         -- &          0 &            &          0 &         -- &       0.26 &       0.25 &          7 \\ 
   CS~22886-044 &    SG &       5730 &       3.75 &      -1.86 &      -1.65 &          0 &         -- &      -0.01 &       0.24 &          3 &            &          0 &         -- &       0.12 &       0.22 &          7 \\ 
   CS~22888-002 &    SG &       5700 &       3.50 &      -2.93 &      -2.91 &          1 &   4389.979 &       0.40 &         -- &          0 &            &          0 &         -- &       0.49 &       0.33 &          1 \\ 
   CS~22888-014 &    SG &       6020 &       3.70 &      -2.73 &      -2.69 &          1 &   4389.979 &       0.63 &         -- &          0 &            &          0 &         -- &       0.35 &       0.24 &          3 \\ 
   CS~22888-031 &    SG &       5810 &       3.50 &      -3.71 &      -3.41 &          1 &    4379.23 &       1.36 &         -- &          0 &            &          1 &   3715.464 &       1.02 &         -- &          0 \\ 
   CS~22888-047 &    HB &       5950 &       1.90 &      -2.54 &      -2.54 &          0 &         -- &      -0.24 &       0.22 &          1 &            &          0 &         -- &       0.01 &       0.21 &          7 \\ 
   CS~22889-050 &    SG &       5920 &       3.60 &      -3.09 &      -2.84 &          1 &    4379.23 &       0.94 &         -- &          0 &            &          0 &         -- &       0.39 &       0.22 &          2 \\ 
   CS~22890-011 &    SG &       6010 &       3.70 &      -2.68 &      -2.47 &          0 &         -- &       0.15 &       0.22 &          1 &            &          0 &         -- &       0.27 &       0.22 &          4 \\ 
   CS~22890-024 &    RG &       5320 &       2.95 &      -2.77 &      -2.58 &          0 &         -- &      -0.07 &        0.10 &          3 &            &          0 &         -- &      -0.01 &        0.20 &          6 \\ 
   CS~22890-064 &    SG &       5960 &       3.60 &      -3.12 &      -3.20 &          1 &   4111.779 &       1.22 &         -- &          0 &            &          1 &   4005.702 &       1.00 &         -- &          0 \\ 
   CS~22891-184 &    HB &       5530 &       1.60 &      -2.68 &      -2.67 &          0 &         -- &      -0.14 &       0.31 &          1 &            &          0 &         -- &      -0.13 &       0.22 &          6 \\ 
   CS~22891-200 &    RG &       4490 &       0.50 &      -4.06 &      -3.88 &          1 &   4389.979 &       0.14 &         -- &          0 &            &          0 &         -- &      -0.02 &        0.20 &          3 \\ 
   CS~22891-209 &    RG &       4620 &       0.95 &      -3.49 &      -3.26 &          0 &         -- &       0.01 &       0.11 &          3 &            &          0 &         -- &       0.07 &       0.22 &          7 \\ 
   CS~22891-221 &    RG &       5290 &       2.80 &      -3.23 &      -3.48 &          0 &         -- &      -0.07 &       0.31 &          1 &            &          1 &   3715.464 &       0.60 &         -- &          0 \\ 
   CS~22892-025 &    SG &       6140 &       3.75 &      -2.78 &      -2.66 &          1 &   4111.779 &       1.11 &         -- &          0 &            &          0 &         -- &       0.42 &       0.22 &          3 \\ 
   CS~22892-052 &    RG &       4690 &       1.15 &      -3.24 &      -3.16 &          0 &         -- &      -0.37 &        0.10 &          2 &            &          0 &         -- &      -0.15 &       0.19 &          7 \\ 
   CS~22893-005 &    RG &       5260 &       2.75 &      -2.99 &      -2.93 &          0 &         -- &       0.18 &       0.15 &          2 &            &          0 &         -- &       0.27 &       0.21 &          3 \\ 
   CS~22893-010 &    RG &       5150 &       2.45 &      -3.12 &      -2.93 &          1 &    4379.23 &       0.26 &         -- &          0 &            &          0 &         -- &       0.11 &       0.21 &          3 \\ 
   CS~22893-011 &    SG &       6010 &       3.75 &      -2.40 &      -2.27 &          0 &         -- &       0.28 &       0.14 &          1 &            &          0 &         -- &       0.33 &       0.21 &          3 \\ 
   CS~22894-004 &    SG &       5920 &       3.65 &      -2.96 &      -2.65 &          1 &   4111.779 &       0.88 &         -- &          0 &            &          0 &         -- &       0.66 &       0.31 &          1 \\ 
   CS~22894-019 &    SG &       5930 &       3.60 &      -2.98 &      -3.04 &          1 &   4111.779 &       1.04 &         -- &          0 &            &          0 &         -- &       0.68 &       0.31 &          1 \\ 
   CS~22894-023 &    SG &       5980 &       3.65 &      -3.14 &      -2.82 &          1 &    4379.23 &       0.90 &         -- &          0 &            &          0 &         -- &       0.27 &       0.23 &          4 \\ 
   CS~22894-049 &    MS &       5870 &       3.90 &      -2.84 &      -2.83 &          1 &   4111.779 &       0.62 &         -- &          0 &            &          0 &         -- &       0.45 &       0.25 &          1 \\ 
   CS~22896-015 &    RG &       5080 &       2.25 &      -2.85 &      -2.84 &          0 &         -- &      -0.06 &       0.11 &          3 &            &          0 &         -- &       0.03 &       0.22 &          6 \\ 
   CS~22896-055 &    HB &       5970 &       1.85 &      -2.52 &      -2.51 &          1 &   4111.779 &       0.45 &         -- &          0 &            &          0 &         -- &       0.19 &       0.21 &          7 \\ 
   CS~22896-110 &    HB &       5380 &       1.15 &      -2.85 &      -2.86 &          0 &         -- &       0.17 &       0.09 &          2 &            &          0 &         -- &       0.19 &       0.23 &          6 \\ 
   CS~22896-115 &    SG &       5910 &       3.65 &      -2.82 &      -2.72 &          1 &   4111.779 &       0.56 &         -- &          0 &            &          0 &         -- &       0.22 &       0.23 &          2 \\ 
   CS~22896-136 &    SG &       6190 &       3.85 &      -2.41 &      -2.19 &          1 &    4379.23 &       0.36 &         -- &          0 &            &          0 &         -- &       0.22 &       0.21 &          5 \\ 
   CS~22897-008 &    RG &       4550 &       0.70 &      -3.83 &      -3.73 &          0 &         -- &       0.16 &       0.18 &          3 &            &          0 &         -- &       0.20 &       0.18 &          6 \\ 
   CS~22898-043 &    HB &       6160 &       2.15 &      -2.83 &      -2.80 &          1 &   4111.779 &       0.89 &         -- &          0 &            &          0 &         -- &       0.33 &       0.22 &          4 \\ 
   CS~22898-047 &    RG &       5150 &       2.40 &      -3.51 &      -3.45 &          0 &         -- &       0.05 &       0.22 &          1 &            &          0 &         -- &       0.16 &       0.21 &          4 \\ 
   CS~22937-072 &    HB &       5500 &       1.75 &      -2.72 &      -2.71 &          0 &         -- &       0.23 &       0.18 &          3 &            &          0 &         -- &       0.23 &        0.20 &          7 \\ 
   CS~22940-070 &    HB &       6130 &       1.85 &      -1.43 &      -1.46 &          0 &         -- &      -0.05 &        0.10 &          4 &            &          0 &         -- &       0.11 &       0.21 &          6 \\ 
   CS~22940-077 &    HB &       5350 &       1.35 &      -3.10 &      -3.10 &          0 &         -- &       0.49 &       0.18 &          1 &            &          0 &         -- &       0.16 &       0.22 &          6 \\ 
   CS~22940-121 &    HB &       5200 &       1.15 &      -3.14 &      -3.13 &          0 &         -- &       0.33 &       0.13 &          1 &            &          0 &         -- &       0.19 &        0.20 &          6 \\ 
   CS~22941-017 &    RG &       5070 &       2.20 &      -3.11 &      -3.08 &          0 &         -- &       0.06 &       0.12 &          2 &            &          0 &         -- &       0.19 &       0.21 &          6 \\ 
   CS~22941-027 &    HB &       6050 &       1.70 &      -2.71 &      -2.71 &          1 &   4111.779 &       0.47 &         -- &          0 &            &          0 &         -- &       0.06 &       0.22 &          4 \\ 
   CS~22942-002 &    RG &       5010 &       2.00 &      -3.61 &      -3.53 &          0 &         -- &      -0.16 &       0.32 &          1 &            &          0 &         -- &       0.03 &       0.27 &          5 \\ 
   CS~22942-011 &    RG &       4930 &       1.85 &      -2.88 &      -2.83 &          0 &         -- &      -0.34 &       0.09 &          3 &            &          0 &         -- &       0.04 &       0.19 &          6 \\ 
   CS~22942-035 &    RG &       4940 &       1.85 &      -3.08 &      -2.99 &          0 &         -- &      -0.12 &        0.10 &          3 &            &          0 &         -- &       0.03 &       0.22 &          6 \\ 
   CS~22943-059 &    SG &       5810 &       3.60 &      -2.95 &      -2.64 &          1 &    4379.23 &       0.71 &         -- &          0 &            &          0 &         -- &       0.25 &       0.22 &          4 \\ 
   CS~22943-095 &    SG &       6140 &       3.80 &      -2.52 &      -2.44 &          0 &         -- &       0.09 &       0.14 &          1 &            &          0 &         -- &       0.28 &       0.23 &          5 \\ 
   CS~22943-132 &    SG &       5850 &       3.60 &      -2.63 &      -2.67 &          0 &         -- &       0.19 &       0.13 &          2 &            &          0 &         -- &       0.15 &       0.29 &          6 \\ 
   CS~22943-137 &    RG &       5400 &       3.10 &      -3.64 &      -3.39 &          1 &    4379.23 &       1.04 &         -- &          0 &            &          1 &   3545.196 &       0.82 &         -- &          0 \\ 
   CS~22943-201 &    HB &       5970 &       2.45 &      -2.68 &      -2.69 &          1 &    4379.23 &       0.45 &         -- &          0 &            &          0 &         -- &       0.14 &       0.26 &          3 \\ 
   CS~22944-014 &    SG &       6020 &       3.70 &      -2.64 &      -2.62 &          1 &    4379.23 &       0.30 &         -- &          0 &            &          0 &         -- &       0.35 &       0.23 &          3 \\ 
   CS~22944-032 &    RG &       5090 &       2.30 &      -3.22 &      -3.15 &          0 &         -- &       0.09 &        0.10 &          3 &            &          0 &         -- &       0.11 &       0.23 &          6 \\ 
   CS~22944-061 &    SG &       5920 &       3.60 &      -2.96 &      -2.95 &          1 &   4111.779 &       0.75 &         -- &          0 &            &          0 &         -- &       0.40 &        0.30 &          1 \\ 
   CS~22945-017 &    SG &       6080 &       3.70 &      -2.89 &      -2.73 &          1 &    4379.23 &       0.44 &         -- &          0 &            &          1 &   4005.702 &       0.58 &         -- &          0 \\ 
   CS~22945-024 &    RG &       5120 &       2.35 &      -2.58 &      -2.59 &          0 &         -- &      -0.01 &       0.13 &          1 &            &          0 &         -- &       0.14 &       0.21 &          5 \\ 
   CS~22945-028 &    RG &       4900 &       1.75 &      -2.92 &      -2.89 &          0 &         -- &      -0.07 &       0.12 &          3 &            &          0 &         -- &      -0.04 &       0.23 &          6 \\ 
   CS~22945-031 &    SG &       5820 &       3.55 &      -3.29 &      -3.03 &          1 &   4111.779 &       1.24 &         -- &          0 &            &          1 &   4023.377 &       0.68 &         -- &          0 \\ 
   CS~22945-056 &    HB &       6000 &       1.75 &      -2.82 &      -2.83 &          1 &    4379.23 &       0.76 &         -- &          0 &            &          0 &         -- &       0.14 &       0.24 &          4 \\ 
   CS~22945-058 &    SG &       5990 &       3.65 &      -2.98 &      -2.71 &          1 &   4111.779 &       0.97 &         -- &          0 &            &          0 &         -- &       0.49 &       0.25 &          1 \\ 
   CS~22945-063 &    HB &       5730 &       1.70 &      -2.84 &      -2.84 &          0 &         -- &       0.10 &       0.13 &          1 &            &          0 &         -- &       0.30 &       0.21 &          6 \\ 
   CS~22947-187 &    HB &       5300 &       1.40 &      -2.58 &      -2.58 &          0 &         -- &      -0.05 &       0.09 &          3 &            &          0 &         -- &       0.15 &       0.23 &          7 \\ 
   CS~22948-066 &    RG &       4830 &       1.55 &      -3.50 &      -3.18 &          0 &         -- &       0.33 &       0.17 &          2 &            &          0 &         -- &       0.23 &        0.20 &          6 \\ 
   CS~22948-093 &    SG &       6540 &       3.85 &      -3.32 &      -3.42 &          1 &    4379.23 &       1.45 &         -- &          0 &            &          1 &   3715.464 &       1.20 &         -- &          0 \\ 
   CS~22949-030 &    SG &       5890 &       3.60 &      -3.01 &      -2.88 &          1 &   4111.779 &       0.57 &         -- &          0 &            &          0 &         -- &       0.28 &       0.22 &          2 \\ 
   CS~22949-037 &    RG &       4630 &       0.95 &      -4.38 &      -4.20 &          0 &         -- &       0.45 &        0.10 &          2 &            &          0 &         -- &       0.47 &       0.23 &          3 \\ 
   CS~22949-048 &    RG &       4620 &       0.95 &      -3.55 &      -3.37 &          0 &         -- &      -0.13 &       0.11 &          3 &            &          0 &         -- &       0.01 &       0.21 &          6 \\ 
   CS~22950-046 &    RG &       4380 &       0.50 &      -4.12 &      -3.64 &          0 &         -- &      -0.12 &       0.22 &          1 &            &          0 &         -- &      -0.11 &        0.20 &          5 \\ 
   CS~22951-005 &    SG &       5950 &       3.65 &      -2.74 &      -2.67 &          1 &    4379.23 &       0.69 &         -- &          0 &            &          0 &         -- &       0.25 &       0.28 &          5 \\ 
   CS~22951-059 &    RG &       5120 &       2.35 &      -2.84 &      -2.83 &          0 &         -- &      -0.12 &        0.10 &          2 &            &          0 &         -- &       0.15 &       0.22 &          5 \\ 
   CS~22951-077 &    HB &       5290 &       1.45 &      -2.54 &      -2.54 &          0 &         -- &      -0.09 &        0.10 &          4 &            &          0 &         -- &       0.01 &       0.23 &          7 \\ 
   CS~22952-015 &    RG &       4500 &       0.55 &      -3.87 &      -3.68 &          0 &         -- &      -0.08 &       0.22 &          1 &            &          0 &         -- &      -0.20 &       0.22 &          5 \\ 
   CS~22953-003 &    RG &       4860 &       1.65 &      -3.13 &      -3.00 &          0 &         -- &      -0.26 &       0.14 &          3 &            &          0 &         -- &      -0.09 &       0.19 &          6 \\ 
   CS~22953-037 &    SG &       6150 &       3.70 &      -3.21 &      -3.05 &          1 &   4111.779 &       1.14 &         -- &          0 &            &          1 &   3715.464 &       0.78 &         -- &          0 \\ 
   CS~22954-004 &    SG &       5810 &       3.55 &      -3.00 &      -2.78 &          1 &    4379.23 &       0.66 &         -- &          0 &            &          0 &         -- &       0.25 &       0.22 &          2 \\ 
   CS~22954-015 &    SG &       5930 &       3.75 &      -2.11 &      -1.97 &          0 &         -- &       0.10 &       0.22 &          1 &            &          0 &         -- &       0.28 &       0.22 &          6 \\ 
   CS~22955-110 &    BS &       6710 &       3.45 &      -1.37 &      -1.39 &          0 &         -- &       0.16 &       0.12 &          3 &            &          0 &         -- &       0.13 &       0.13 &          7 \\ 
   CS~22955-174 &    HB &       5520 &       1.35 &      -3.10 &      -3.10 &          1 &   4111.779 &       0.42 &         -- &          0 &            &          0 &         -- &       0.26 &       0.23 &          5 \\ 
   CS~22956-015 &    SG &       5960 &       3.70 &      -2.81 &      -2.48 &          1 &   4389.979 &       0.57 &         -- &          0 &            &          0 &         -- &       0.23 &       0.22 &          2 \\ 
   CS~22956-021 &    SG &       6020 &       3.70 &      -2.73 &      -2.51 &          1 &   4111.779 &       0.66 &         -- &          0 &            &          0 &         -- &       0.22 &       0.22 &          4 \\ 
   CS~22956-050 &    RG &       4640 &       1.00 &      -3.67 &      -3.57 &          0 &         -- &      -0.19 &       0.16 &          2 &            &          0 &         -- &       0.21 &       0.23 &          6 \\ 
   CS~22956-062 &    SG &       5540 &       3.40 &      -2.75 &      -2.76 &          0 &         -- &      -0.10 &       0.12 &          2 &            &          0 &         -- &       0.46 &       0.23 &          3 \\ 
   CS~22956-081 &    SG &       6310 &       3.80 &      -2.71 &      -2.80 &          1 &    4379.23 &       0.80 &         -- &          0 &            &          1 &   3715.464 &       1.14 &         -- &          0 \\ 
   CS~22956-102 &    SG &       6220 &       3.85 &      -2.39 &      -2.21 &          1 &    4379.23 &       0.57 &         -- &          0 &            &          0 &         -- &       0.42 &       0.24 &          1 \\ 
   CS~22956-106 &    SG &       6410 &       3.90 &      -2.69 &      -2.60 &          1 &   4111.779 &       1.16 &         -- &          0 &            &          1 &   3545.196 &       0.87 &         -- &          0 \\ 
   CS~22956-110 &    HB &       6010 &       1.85 &      -3.15 &      -3.14 &          1 &    4379.23 &       0.84 &         -- &          0 &            &          0 &         -- &       0.58 &       0.24 &          3 \\ 
   CS~22956-114 &    RG &       4900 &       1.75 &      -3.19 &      -2.86 &          0 &         -- &      -0.11 &       0.09 &          2 &            &          0 &         -- &      -0.03 &       0.23 &          6 \\ 
   CS~22957-013 &    RG &       4620 &       0.95 &      -2.98 &      -3.01 &          0 &         -- &      -0.33 &       0.13 &          2 &            &          0 &         -- &       0.05 &        0.20 &          7 \\ 
   CS~22957-019 &    SG &       6070 &       3.75 &      -2.43 &      -2.42 &          0 &         -- &       0.12 &       0.22 &          1 &            &          0 &         -- &       0.18 &       0.24 &          6 \\ 
   CS~22957-022 &    RG &       4860 &       1.65 &      -3.28 &      -3.17 &          0 &         -- &      -0.04 &       0.11 &          3 &            &          0 &         -- &       0.03 &       0.22 &          6 \\ 
   CS~22957-024 &    SG &       6160 &       3.75 &      -2.91 &      -2.81 &          1 &    4379.23 &       0.90 &         -- &          0 &            &          0 &         -- &       0.77 &       0.25 &          1 \\ 
   CS~22957-026 &    SG &       6120 &       3.90 &      -1.93 &      -1.89 &          0 &         -- &       0.02 &       0.11 &          2 &            &          0 &         -- &       0.13 &       0.22 &          7 \\ 
   CS~22957-027 &    RG &       5220 &       2.65 &      -3.19 &      -3.00 &          1 &    4379.23 &       1.23 &         -- &          0 &            &          0 &         -- &       0.27 &       0.19 &          3 \\ 
   CS~22957-036 &    SG &       5970 &       3.75 &      -2.28 &      -2.09 &          0 &         -- &       0.14 &       0.31 &          1 &            &          0 &         -- &       0.19 &       0.21 &          6 \\ 
   CS~22958-037 &    HB &       5770 &       2.10 &      -2.51 &      -2.51 &          0 &         -- &       0.12 &       0.13 &          1 &            &          0 &         -- &       0.20 &       0.23 &          6 \\ 
   CS~22958-041 &    SG &       6010 &       3.65 &      -3.10 &      -2.88 &          1 &    4379.23 &       1.32 &         -- &          0 &            &          1 &   3715.464 &       0.96 &         -- &          0 \\ 
   CS~22958-042 &    SG &       5760 &       3.55 &      -3.40 &      -2.99 &          1 &    4379.23 &       0.90 &         -- &          0 &            &          1 &   3715.464 &       0.60 &         -- &          0 \\ 
   CS~22958-052 &    SG &       6090 &       3.75 &      -2.62 &      -2.42 &          1 &   4111.779 &       0.72 &         -- &          0 &            &          0 &         -- &       0.37 &       0.22 &          3 \\ 
   CS~22958-065 &    SG &       6020 &       3.75 &      -2.29 &      -2.24 &          0 &         -- &       0.07 &       0.18 &          1 &            &          0 &         -- &       0.13 &       0.25 &          5 \\ 
   CS~22958-074 &    SG &       5800 &       3.60 &      -2.67 &      -2.62 &          1 &    4379.23 &       0.50 &         -- &          0 &            &          0 &         -- &       0.34 &       0.23 &          2 \\ 
   CS~22958-083 &    RG &       4900 &       1.75 &      -3.05 &      -3.04 &          0 &         -- &      -0.09 &       0.11 &          3 &            &          0 &         -- &       0.05 &        0.20 &          7 \\ 
   CS~22959-074 &    RG &       4940 &       1.90 &      -2.60 &      -2.49 &          0 &         -- &      -0.30 &       0.09 &          4 &            &          0 &         -- &      -0.05 &       0.21 &          7 \\ 
   CS~22959-139 &    SG &       6090 &       3.75 &      -2.67 &      -2.45 &          1 &    4379.23 &       0.76 &         -- &          0 &            &          0 &         -- &       0.54 &       0.29 &          1 \\ 
   CS~22960-010 &    MS &       5280 &       4.00 &      -3.02 &      -3.03 &          0 &         -- &      -0.21 &       0.11 &          1 &            &          0 &         -- &       0.56 &       0.15 &          2 \\ 
   CS~22960-029 &    SG &       5890 &       3.60 &      -3.05 &      -2.77 &          1 &   4389.979 &       0.72 &         -- &          0 &            &          1 &   3545.196 &       0.58 &         -- &          0 \\ 
   CS~22960-048 &    RG &       4770 &       1.40 &      -3.91 &      -3.78 &          0 &         -- &       0.51 &       0.22 &          1 &            &          0 &         -- &       0.21 &       0.19 &          3 \\ 
   CS~22960-053 &    RG &       4860 &       1.65 &      -3.64 &      -3.33 &          1 &    4379.23 &       0.45 &         -- &          0 &            &          1 &   3517.299 &       0.68 &         -- &          0 \\ 
   CS~22960-064 &    RG &       5060 &       2.20 &      -2.77 &      -2.77 &          0 &         -- &      -0.16 &       0.09 &          3 &            &          0 &         -- &       0.11 &        0.20 &          7 \\ 
   CS~22963-004 &    RG &       5060 &       2.15 &      -4.09 &      -3.85 &          1 &    4379.23 &       1.11 &         -- &          0 &            &          1 &   4005.702 &       0.57 &         -- &          0 \\ 
   CS~22964-115 &    SG &       6090 &       3.70 &      -2.82 &      -2.70 &          1 &   4389.979 &       0.85 &         -- &          0 &            &          0 &         -- &       0.51 &       0.25 &          1 \\ 
   CS~22964-176 &    SG &       6000 &       3.70 &      -2.56 &      -2.46 &          1 &   4111.779 &       0.77 &         -- &          0 &            &          0 &         -- &       0.29 &       0.23 &          5 \\ 
   CS~22964-183 &    SG &       6010 &       3.65 &      -3.01 &      -2.87 &          1 &    4379.23 &       0.94 &         -- &          0 &            &          1 &   3715.464 &       0.76 &         -- &          0 \\ 
   CS~22964-214 &    SG &       6180 &       3.75 &      -2.95 &      -2.84 &          1 &    4379.23 &       0.86 &         -- &          0 &            &          1 &   3517.299 &       0.61 &         -- &          0 \\ 
   CS~22965-016 &    RG &       4770 &       1.40 &      -3.13 &      -2.93 &          0 &         -- &      -0.02 &       0.13 &          3 &            &          0 &         -- &       0.13 &        0.20 &          4 \\ 
   CS~22965-054 &    SG &       6050 &       3.70 &      -3.17 &      -2.89 &          1 &    4379.23 &       1.38 &         -- &          0 &            &          1 &   3715.464 &       0.26 &         -- &          0 \\ 
   CS~22968-001 &    SG &       5940 &       3.65 &      -3.12 &      -2.84 &          1 &   4111.779 &       1.05 &         -- &          0 &            &          0 &         -- &       0.38 &       0.38 &          1 \\ 
   CS~22968-014 &    RG &       4540 &       0.60 &      -3.99 &      -3.85 &          0 &         -- &       0.03 &       0.22 &          1 &            &          0 &         -- &      -0.08 &        0.20 &          3 \\ 
   CS~22968-026 &    SG &       5850 &       3.65 &      -2.57 &      -2.33 &          0 &         -- &       0.02 &       0.12 &          2 &            &          0 &         -- &       0.20 &       0.22 &          4 \\ 
   CS~22968-029 &    SG &       5760 &       3.50 &      -3.10 &      -3.11 &          1 &    4379.23 &       0.93 &         -- &          0 &            &          1 &   3951.957 &       0.86 &         -- &          0 \\ 
   CS~29493-023 &    SG &       5980 &       3.65 &      -2.89 &      -2.66 &          1 &    4379.23 &       0.83 &         -- &          0 &            &          0 &         -- &       0.28 &       0.37 &          1 \\ 
   CS~29493-050 &    SG &       6270 &       3.80 &      -2.92 &      -2.89 &          1 &    4379.23 &       1.17 &         -- &          0 &            &          0 &         -- &       0.41 &        0.30 &          1 \\ 
   CS~29493-062 &    SG &       5520 &       3.40 &      -2.76 &      -2.59 &          0 &         -- &       0.08 &       0.32 &          1 &            &          0 &         -- &       0.18 &       0.23 &          5 \\ 
   CS~29493-094 &    SG &       6130 &       3.80 &      -2.66 &      -2.44 &          1 &   4111.779 &       0.91 &         -- &          0 &            &          1 &   3715.464 &       0.19 &         -- &          0 \\ 
   CS~29495-005 &    SG &       5990 &       3.75 &      -2.44 &      -2.26 &          0 &         -- &       0.08 &       0.13 &          1 &            &          0 &         -- &       0.26 &       0.22 &          6 \\ 
   CS~29495-042 &    RG &       5180 &       2.55 &      -2.54 &      -2.18 &          1 &   4111.779 &      -0.10 &         -- &          0 &            &          0 &         -- &      -0.02 &       0.26 &          7 \\ 
   CS~29497-030 &    BS &       7000 &       4.00 &      -2.52 &      -2.52 &          1 &    4379.23 &       1.32 &         -- &          0 &            &          0 &         -- &       0.72 &       0.43 &          1 \\ 
   CS~29498-043 &    RG &       4440 &       0.50 &      -3.87 &      -3.85 &          1 &    4379.23 &       0.51 &         -- &          0 &            &          0 &         -- &       0.20 &       0.31 &          1 \\ 
   CS~29499-003 &    SG &       6080 &       3.75 &      -2.51 &      -2.35 &          1 &    4379.23 &       0.52 &         -- &          0 &            &          0 &         -- &       0.36 &       0.25 &          5 \\ 
   CS~29499-058 &    SG &       6060 &       3.70 &      -2.81 &      -2.61 &          1 &    4379.23 &       0.86 &         -- &          0 &            &          0 &         -- &       0.31 &       0.22 &          4 \\ 
   CS~29499-060 &    SG &       6280 &       3.80 &      -2.79 &      -2.75 &          1 &    4379.23 &       1.06 &         -- &          0 &            &          0 &         -- &       0.46 &       0.22 &          2 \\ 
   CS~29501-032 &    SG &       5950 &       3.65 &      -2.92 &      -2.71 &          1 &    4379.23 &       0.71 &         -- &          0 &            &          1 &   4023.377 &       0.50 &         -- &          0 \\ 
   CS~29502-092 &    RG &       4820 &       1.50 &      -3.30 &      -3.20 &          1 &   4111.779 &       0.05 &         -- &          0 &            &          0 &         -- &      -0.04 &       0.21 &          6 \\ 
   CS~29504-004 &    HB &       7500 &       2.50 &      -2.38 &      -2.35 &          1 &    4379.23 &       1.75 &         -- &          0 &            &          1 &   4005.702 &       0.37 &         -- &          0 \\ 
   CS~29504-006 &    SG &       6150 &       3.70 &      -3.12 &      -2.91 &          1 &   4111.779 &       1.41 &         -- &          0 &            &          1 &   4023.377 &       1.20 &         -- &          0 \\ 
   CS~29506-007 &    SG &       5940 &       3.60 &      -3.24 &      -2.94 &          1 &   4111.779 &       1.21 &         -- &          0 &            &          0 &         -- &       0.31 &       0.24 &          1 \\ 
   CS~29506-090 &    SG &       5940 &       3.60 &      -3.21 &      -3.08 &          1 &   4111.779 &       1.14 &         -- &          0 &            &          1 &   3715.464 &       0.82 &         -- &          0 \\ 
   CS~29509-027 &    BS &       6850 &       3.50 &      -2.42 &      -2.42 &          1 &   4389.979 &       0.73 &         -- &          0 &            &          0 &         -- &       0.19 &       0.15 &          6 \\ 
   CS~29512-073 &    SG &       5650 &       3.60 &      -2.10 &      -1.93 &          1 &    4379.23 &      -0.10 &         -- &          0 &            &          0 &         -- &      -0.25 &       0.27 &          7 \\ 
   CS~29513-003 &    HB &       5480 &       1.90 &      -2.47 &      -2.46 &          0 &         -- &       0.08 &       0.12 &          2 &            &          0 &         -- &       0.10 &       0.21 &          6 \\ 
   CS~29513-014 &    HB &       5440 &       1.55 &      -2.32 &      -2.32 &          0 &         -- &      -0.01 &       0.09 &          2 &            &          0 &         -- &       0.08 &       0.21 &          7 \\ 
   CS~29513-015 &    SG &       6110 &       3.75 &      -2.63 &      -2.51 &          1 &    4379.23 &       0.60 &         -- &          0 &            &          0 &         -- &       0.00 &       0.24 &          1 \\ 
   CS~29513-031 &    SG &       6600 &       4.00 &      -2.67 &      -2.59 &          1 &    4379.23 &       1.18 &         -- &          0 &            &          1 &   3517.299 &       0.29 &         -- &          0 \\ 
   CS~29513-032 &    SG &       6080 &       3.85 &      -1.85 &      -1.91 &          0 &         -- &      -0.03 &       0.12 &          1 &            &          0 &         -- &       0.12 &       0.27 &          5 \\ 
   CS~29514-007 &    SG &       6400 &       3.85 &      -2.83 &      -2.81 &          1 &    4379.23 &       1.20 &         -- &          0 &            &          1 &   4005.702 &       0.88 &         -- &          0 \\ 
   CS~29514-017 &    RG &       5270 &       2.80 &      -2.35 &      -2.34 &          0 &         -- &      -0.26 &       0.13 &          3 &            &          0 &         -- &      -0.06 &       0.26 &          6 \\ 
   CS~29514-018 &    SG &       5990 &       3.70 &      -2.84 &      -2.58 &          1 &    4379.23 &       0.40 &         -- &          0 &            &          0 &         -- &       0.19 &       0.24 &          4 \\ 
   CS~29514-037 &    SG &       5970 &       3.70 &      -2.62 &      -2.47 &          0 &         -- &       0.35 &       0.12 &          1 &            &          0 &         -- &       0.12 &       0.22 &          5 \\ 
   CS~29517-018 &    SG &       5680 &       3.50 &      -2.78 &      -2.94 &          0 &         -- &       0.14 &       0.19 &          1 &            &          0 &         -- &       0.52 &       0.22 &          2 \\ 
   CS~29517-042 &    SG &       6120 &       3.75 &      -2.53 &      -2.54 &          1 &   4111.779 &       0.64 &         -- &          0 &            &          0 &         -- &       0.26 &       0.24 &          4 \\ 
   CS~29529-054 &    SG &       5710 &       3.55 &      -2.55 &      -2.75 &          0 &         -- &      -0.03 &       0.14 &          1 &            &          1 &   4005.702 &       0.56 &         -- &          0 \\ 
   CS~30312-044 &    RG &       4660 &       1.05 &      -3.22 &      -3.19 &          0 &         -- &      -0.12 &        0.10 &          3 &            &          0 &         -- &      -0.02 &       0.19 &          5 \\ 
   CS~30312-059 &    RG &       4780 &       1.40 &      -3.41 &      -3.26 &          0 &         -- &      -0.22 &       0.11 &          3 &            &          0 &         -- &      -0.05 &       0.19 &          6 \\ 
   CS~30312-062 &    HB &       6600 &       2.45 &      -2.64 &      -2.65 &          1 &   4111.779 &       0.84 &         -- &          0 &            &          0 &         -- &       0.19 &       0.21 &          3 \\ 
   CS~30312-100 &    RG &       5040 &       2.15 &      -2.69 &      -2.68 &          0 &         -- &      -0.04 &       0.09 &          3 &            &          0 &         -- &       0.22 &        0.20 &          7 \\ 
   CS~30314-067 &    RG &       4320 &       0.50 &      -3.31 &      -3.01 &          0 &         -- &      -0.43 &       0.12 &          3 &            &          0 &         -- &      -0.01 &       0.21 &          7 \\ 
   CS~30339-015 &    SG &       5840 &       3.60 &      -3.00 &      -2.86 &          1 &   4111.779 &       0.59 &         -- &          0 &            &          1 &   4005.702 &       0.45 &         -- &          0 \\ 
   CS~30339-046 &    HB &       7000 &       2.55 &      -2.71 &      -2.69 &          1 &   4111.779 &       1.27 &         -- &          0 &            &          1 &   4005.702 &       0.35 &         -- &          0 \\ 
   CS~30339-052 &    HB &       5580 &       2.35 &      -2.69 &      -2.67 &          1 &   4111.779 &       0.55 &         -- &          0 &            &          0 &         -- &       0.18 &       0.25 &          3 \\ 
   CS~30339-069 &    SG &       5900 &       3.55 &      -3.50 &      -3.17 &          1 &    4379.23 &       1.15 &         -- &          0 &            &          1 &   4005.702 &       0.52 &         -- &          0 \\ 
   CS~30339-073 &    RG &       4830 &       1.55 &      -3.93 &      -3.80 &          1 &    4379.23 &       0.76 &         -- &          0 &            &          0 &         -- &       0.42 &       0.36 &          1 \\ 
   CS~30492-001 &    SG &       5790 &       3.65 &      -2.62 &      -2.35 &          0 &         -- &       0.15 &       0.18 &          1 &            &          0 &         -- &       0.26 &       0.22 &          5 \\ 
   CS~30492-016 &    SG &       5570 &       3.35 &      -3.30 &      -3.40 &          1 &   4389.979 &       0.79 &         -- &          0 &            &          1 &   4005.702 &       0.89 &         -- &          0 \\ 
   CS~30492-110 &    RG &       4660 &       1.05 &      -3.27 &      -3.16 &          0 &         -- &      -0.33 &       0.22 &          1 &            &          0 &         -- &      -0.03 &        0.20 &          6 \\ 
   CS~30493-071 &    SG &       5700 &       3.55 &      -2.82 &      -2.46 &          0 &         -- &       0.18 &       0.11 &          1 &            &          0 &         -- &       0.10 &       0.24 &          5 \\ 
   CS~30494-003 &    RG &       4930 &       1.85 &      -2.97 &      -2.97 &          0 &         -- &      -0.21 &       0.09 &          3 &            &          0 &         -- &       0.07 &       0.22 &          6 \\ 
   CS~31082-001 &    RG &       4650 &       1.05 &      -3.09 &      -3.03 &          0 &         -- &      -0.11 &       0.12 &          3 &            &          0 &         -- &      -0.06 &        0.20 &          6 \\ 
       G004-036 &    SG &       5810 &       3.65 &      -2.17 &      -2.22 &          0 &         -- &       0.16 &        0.10 &          2 &            &          0 &         -- &       0.26 &       0.22 &          5 \\ 
       G004-037 &    SG &       6110 &       3.75 &      -2.73 &      -2.67 &          1 &    4379.23 &       0.81 &         -- &          0 &            &          1 &   3951.957 &       0.50 &         -- &          0 \\ 
       G009-027 &    MS &       5360 &       4.15 &      -1.79 &      -1.81 &          0 &         -- &      -0.23 &        0.10 &          2 &            &          1 &   4005.702 &       0.39 &         -- &          0 \\ 
       G010-054 &    MS &       5210 &       4.40 &      -2.29 &      -2.30 &          0 &         -- &      -0.08 &       0.14 &          2 &            &          1 &   3951.957 &       0.48 &         -- &          0 \\ 
       G015-010 &    MS &       5050 &       4.05 &      -2.53 &      -2.54 &          0 &         -- &      -0.17 &       0.09 &          3 &            &          0 &         -- &       0.16 &       0.17 &          5 \\ 
       G016-025 &    MS &       5250 &       4.10 &      -2.08 &      -2.07 &          0 &         -- &      -0.32 &       0.12 &          2 &            &          1 &   4023.377 &       0.16 &         -- &          0 \\ 
       G025-022 &    MS &       5350 &       3.95 &      -2.33 &      -2.33 &          0 &         -- &      -0.14 &       0.15 &          2 &            &          1 &   4005.702 &       0.54 &         -- &          0 \\ 
       G025-024 &    SG &       5670 &       3.55 &      -2.11 &      -2.28 &          0 &         -- &      -0.09 &       0.19 &          1 &            &          0 &         -- &       0.23 &       0.24 &          1 \\ 
       G026-001 &    SG &       5860 &       3.75 &      -2.08 &      -1.94 &          0 &         -- &       0.02 &       0.14 &          2 &            &          0 &         -- &       0.16 &       0.23 &          5 \\ 
       G064-012 &    SG &       6030 &       3.60 &      -3.58 &      -3.39 &          1 &   4111.779 &       1.42 &         -- &          0 &            &          1 &   3715.464 &       0.74 &         -- &          0 \\ 
       G071-055 &    SG &       5550 &       3.55 &      -2.06 &      -1.82 &          0 &         -- &      -0.16 &       0.14 &          4 &            &          0 &         -- &       0.08 &       0.23 &          5 \\ 
       G075-056 &    SG &       6190 &       3.85 &      -2.35 &      -2.30 &          1 &    4379.23 &       0.42 &         -- &          0 &            &          0 &         -- &       0.36 &       0.22 &          2 \\ 
       G088-023 &    MS &       5640 &       3.95 &      -1.94 &      -1.94 &          0 &         -- &      -0.13 &       0.18 &          4 &            &          0 &         -- &       0.34 &       0.34 &          1 \\ 
       G090-003 &    SG &       5680 &       3.60 &      -2.40 &      -2.24 &          0 &         -- &      -0.01 &        0.10 &          3 &            &          0 &         -- &       0.14 &       0.22 &          4 \\ 
       G090-025 &    MS &       5150 &       4.05 &      -2.03 &      -2.04 &          0 &         -- &      -0.12 &       0.11 &          3 &            &          0 &         -- &       0.04 &       0.14 &          5 \\ 
       G107-050 &    SG &       6030 &       3.85 &      -2.06 &      -1.89 &          1 &    4379.23 &       0.31 &         -- &          0 &            &          1 &   4005.702 &       0.84 &         -- &          0 \\ 
       G115-049 &    MS &       5420 &       3.80 &      -2.61 &      -2.60 &          0 &         -- &      -0.07 &       0.19 &          1 &            &          1 &   4005.702 &       0.52 &         -- &          0 \\ 
       G122-069 &    SG &       6010 &       3.70 &      -2.78 &      -2.50 &          1 &    4379.23 &       1.04 &         -- &          0 &            &          1 &   3951.957 &       0.52 &         -- &          0 \\ 
       G126-062 &    SG &       5970 &       3.85 &      -1.80 &      -1.70 &          0 &         -- &       0.02 &       0.11 &          4 &            &          0 &         -- &       0.11 &       0.23 &          5 \\ 
       G137-086 &    SG &       5820 &       3.75 &      -1.90 &      -1.76 &          0 &         -- &      -0.11 &       0.19 &          1 &            &          0 &         -- &      -0.13 &       0.25 &          1 \\ 
       G146-056 &    MS &       5290 &       4.05 &      -1.58 &      -1.57 &          0 &         -- &      -0.10 &       0.17 &          4 &            &          1 &   4023.377 &       0.51 &         -- &          0 \\ 
       G146-076 &    RG &       4980 &       2.10 &      -2.08 &      -2.13 &          0 &         -- &      -0.27 &       0.14 &          3 &            &          0 &         -- &      -0.03 &       0.18 &          4 \\ 
       G153-064 &    MS &       5630 &       4.15 &      -1.08 &      -1.09 &          0 &         -- &      -0.12 &       0.11 &          3 &            &          0 &         -- &       0.10 &       0.13 &          5 \\ 
       G161-073 &    SG &       5680 &       3.90 &      -1.42 &      -1.07 &          0 &         -- &      -0.27 &        0.10 &          3 &            &          0 &         -- &      -0.12 &       0.21 &          5 \\ 
       G166-047 &    SG &       5960 &       3.70 &      -2.46 &      -2.28 &          1 &    4379.23 &       0.61 &         -- &          0 &            &          1 &   4005.702 &       0.73 &         -- &          0 \\ 
       G170-047 &    RG &       4930 &       1.85 &      -2.93 &      -2.90 &          0 &         -- &      -0.19 &        0.10 &          3 &            &          0 &         -- &       0.02 &       0.19 &          5 \\ 
       G180-058 &    MS &       4980 &       4.40 &      -2.60 &      -2.62 &          0 &         -- &       0.06 &       0.09 &          2 &            &          0 &         -- &       0.48 &       0.26 &          2 \\ 
       G186-026 &    SG &       5950 &       3.65 &      -3.07 &      -2.90 &          1 &    4379.23 &       0.92 &         -- &          0 &            &          1 &   3951.957 &       0.81 &         -- &          0 \\ 
       G188-022 &    SG &       5890 &       3.90 &      -1.50 &      -1.44 &          0 &         -- &      -0.20 &       0.12 &          4 &            &          0 &         -- &       0.13 &       0.22 &          5 \\ 
       G188-030 &    MS &       5090 &       4.30 &      -2.05 &      -2.07 &          0 &         -- &      -0.03 &       0.14 &          3 &            &          0 &         -- &      -0.12 &       0.18 &          4 \\ 
       G190-010 &    MS &       5230 &       4.35 &      -1.95 &      -1.94 &          0 &         -- &      -0.21 &       0.15 &          4 &            &          0 &         -- &       0.05 &       0.18 &          4 \\ 
       G190-015 &    MS &       4950 &       3.85 &      -3.12 &      -3.13 &          0 &         -- &      -0.04 &        0.10 &          2 &            &          1 &   4023.377 &       0.51 &         -- &          0 \\ 
       G199-066 &    SG &       5560 &       3.45 &      -2.14 &      -2.34 &          0 &         -- &      -0.15 &       0.12 &          2 &            &          0 &         -- &       0.44 &       0.24 &          1 \\ 
       G201-044 &    SG &       6000 &       3.90 &      -1.72 &      -1.63 &          0 &         -- &       0.03 &       0.11 &          2 &            &          0 &         -- &       0.08 &       0.21 &          4 \\ 
       G206-034 &    SG &       5930 &       3.60 &      -3.17 &      -3.13 &          1 &   4111.779 &       0.99 &         -- &          0 &            &          1 &   3951.957 &       0.51 &         -- &          0 \\ 
       G214-001 &    MS &       5370 &       4.05 &      -2.29 &      -2.29 &          0 &         -- &      -0.11 &       0.23 &          2 &            &          1 &   3951.957 &       0.37 &         -- &          0 \\ 
       G234-028 &    SG &       5870 &       3.75 &      -1.80 &      -1.78 &          0 &         -- &      -0.18 &        0.10 &          2 &            &          0 &         -- &       0.07 &       0.22 &          3 \\ 
       G238-030 &    SG &       5740 &       3.50 &      -3.38 &      -3.40 &          1 &    4379.23 &       1.46 &         -- &          0 &            &          1 &   4005.702 &       1.63 &         -- &          0 \\ 
       G238-032 &    MS &       5380 &       4.35 &      -1.59 &      -1.58 &          0 &         -- &      -0.13 &       0.11 &          4 &            &          0 &         -- &       0.28 &       0.15 &          2 \\ 
      HD~106373 &    HB &       6040 &       1.85 &      -2.61 &      -2.60 &          1 &    4379.23 &       0.19 &         -- &          0 &            &          0 &         -- &       0.26 &       0.23 &          6 \\ 
      HD~106373 &    HB &       6040 &       1.85 &      -2.61 &      -2.60 &          1 &   4111.779 &       0.98 &         -- &          0 &            &          0 &         -- &       0.25 &       0.23 &          3 \\ 
      HD~108317 &    RG &       5030 &       2.10 &      -2.62 &      -2.60 &          0 &         -- &      -0.11 &       0.14 &          4 &            &          0 &         -- &       0.17 &       0.18 &          7 \\ 
      HD~108317 &    RG &       5030 &       2.10 &      -2.62 &      -2.60 &          0 &         -- &      -0.28 &       0.11 &          3 &            &          0 &         -- &       0.16 &       0.19 &          4 \\ 
       HD~11582 &    RG &       5020 &       2.20 &      -1.84 &      -2.03 &          0 &         -- &      -0.30 &        0.10 &          4 &            &          0 &         -- &       0.14 &       0.19 &          7 \\ 
      HD~119516 &    HB &       5660 &       1.90 &      -1.94 &      -1.93 &          0 &         -- &      -0.17 &       0.13 &          4 &            &          0 &         -- &      -0.05 &        0.20 &          5 \\ 
      HD~122196 &    SG &       5880 &       3.80 &      -1.97 &      -1.79 &          0 &         -- &      -0.13 &       0.22 &          1 &            &          0 &         -- &       0.05 &       0.24 &          2 \\ 
      HD~122563 &    RG &       4500 &       0.55 &      -2.97 &      -2.93 &          0 &         -- &      -0.21 &       0.09 &          4 &            &          0 &         -- &       0.01 &       0.18 &          4 \\ 
      HD~122563 &    RG &       4500 &       0.55 &      -2.97 &      -2.93 &          0 &         -- &      -0.23 &       0.09 &          4 &            &          0 &         -- &       0.06 &        0.20 &          4 \\ 
      HD~122563 &    RG &       4500 &       0.55 &      -2.97 &      -2.93 &          0 &         -- &      -0.28 &       0.09 &          4 &            &          0 &         -- &       0.08 &       0.18 &          6 \\ 
      HD~126238 &    RG &       4750 &       1.65 &      -2.05 &      -1.96 &          0 &         -- &      -0.40 &        0.10 &          3 &            &          0 &         -- &      -0.13 &       0.18 &          7 \\ 
      HD~126587 &    RG &       4640 &       1.00 &      -3.29 &      -3.21 &          0 &         -- &      -0.11 &        0.10 &          3 &            &          0 &         -- &       0.05 &       0.19 &          7 \\ 
      HD~128279 &    RG &       5050 &       2.15 &      -2.52 &      -2.64 &          0 &         -- &      -0.11 &       0.09 &          3 &            &          0 &         -- &       0.20 &        0.20 &          7 \\ 
      HD~132475 &    SG &       5410 &       3.50 &      -1.82 &      -1.65 &          0 &         -- &      -0.14 &        0.10 &          4 &            &          0 &         -- &       0.14 &       0.22 &          7 \\ 
      HD~132475 &    SG &       5410 &       3.50 &      -1.82 &      -1.65 &          0 &         -- &      -0.18 &       0.12 &          4 &            &          0 &         -- &       0.13 &       0.24 &          5 \\ 
       HD~13979 &    RG &       4830 &       1.60 &      -2.97 &      -2.72 &          0 &         -- &      -0.16 &        0.10 &          4 &            &          0 &         -- &      -0.01 &       0.22 &          7 \\ 
       HD~16031 &    SG &       5870 &       3.75 &      -2.01 &      -1.91 &          0 &         -- &      -0.06 &        0.10 &          2 &            &          0 &         -- &       0.16 &       0.24 &          5 \\ 
      HD~175305 &    RG &       4920 &       2.30 &      -1.63 &      -1.56 &          0 &         -- &      -0.38 &       0.14 &          4 &            &          0 &         -- &      -0.03 &       0.18 &          5 \\ 
      HD~175606 &    SG &       5920 &       3.70 &      -2.39 &      -2.24 &          0 &         -- &      -0.00 &       0.12 &          2 &            &          0 &         -- &       0.15 &       0.23 &          6 \\ 
      HD~178443 &    HB &       5170 &       1.45 &      -1.99 &      -2.02 &          0 &         -- &      -0.11 &        0.10 &          4 &            &          0 &         -- &       0.10 &       0.21 &          7 \\ 
      HD~184266 &    HB &       5780 &       1.85 &      -1.75 &      -1.74 &          0 &         -- &      -0.01 &       0.12 &          3 &            &          0 &         -- &       0.06 &       0.18 &          5 \\ 
      HD~186478 &    RG &       4540 &       0.65 &      -2.75 &      -2.78 &          0 &         -- &      -0.29 &        0.10 &          4 &            &          0 &         -- &       0.04 &       0.18 &          7 \\ 
      HD~188510 &    MS &       5210 &       4.10 &      -1.88 &      -1.88 &          0 &         -- &      -0.20 &        0.10 &          3 &            &          0 &         -- &       0.10 &       0.16 &          5 \\ 
      HD~193901 &    MS &       5580 &       4.05 &      -1.29 &      -1.28 &          0 &         -- &      -0.26 &       0.11 &          4 &            &          0 &         -- &       0.01 &       0.16 &          7 \\ 
       HD~19445 &    SG &       5820 &       3.65 &      -2.29 &      -2.40 &          0 &         -- &       0.03 &       0.18 &          1 &            &          0 &         -- &       0.08 &       0.22 &          4 \\ 
      HD~196892 &    SG &       5670 &       3.85 &      -1.38 &      -1.24 &          0 &         -- &      -0.10 &        0.10 &          3 &            &          0 &         -- &       0.18 &       0.21 &          5 \\ 
      HD~196944 &    HB &       5310 &       1.75 &      -2.39 &      -2.39 &          0 &         -- &      -0.08 &       0.11 &          2 &            &          0 &         -- &      -0.01 &        0.20 &          7 \\ 
      HD~200654 &    RG &       5080 &       2.25 &      -3.13 &      -3.06 &          0 &         -- &      -0.02 &        0.10 &          3 &            &          0 &         -- &       0.11 &        0.20 &          7 \\ 
      HD~201891 &    MS &       5840 &       4.10 &      -1.20 &      -1.21 &          0 &         -- &      -0.14 &       0.13 &          4 &            &          0 &         -- &       0.12 &       0.14 &          5 \\ 
      HD~214362 &    HB &       5760 &       1.65 &      -2.06 &      -2.04 &          0 &         -- &      -0.12 &       0.15 &          3 &            &          0 &         -- &       0.07 &       0.21 &          4 \\ 
       HD~21581 &    RG &       4940 &       2.10 &      -1.70 &      -1.82 &          0 &         -- &      -0.22 &       0.14 &          3 &            &          0 &         -- &       0.19 &       0.18 &          6 \\ 
      HD~219617 &    SG &       5730 &       3.70 &      -1.74 &      -1.83 &          0 &         -- &      -0.08 &       0.11 &          4 &            &          0 &         -- &       0.13 &       0.24 &          5 \\ 
      HD~220127 &    RG &       5060 &       2.40 &      -1.70 &      -1.85 &          0 &         -- &      -0.24 &       0.11 &          3 &            &          0 &         -- &       0.17 &       0.19 &          7 \\ 
      HD~237846 &    RG &       4730 &       1.30 &      -3.21 &      -3.14 &          0 &         -- &      -0.29 &       0.14 &          1 &            &          0 &         -- &      -0.17 &       0.22 &          4 \\ 
       HD~26169 &    RG &       4750 &       1.35 &      -2.80 &      -2.81 &          0 &         -- &      -0.10 &       0.09 &          3 &            &          0 &         -- &       0.09 &       0.18 &          7 \\ 
       HD~26297 &    RG &       4400 &       1.10 &      -1.98 &      -1.72 &          0 &         -- &      -0.44 &       0.17 &          4 &            &          0 &         -- &      -0.00 &        0.20 &          7 \\ 
       HD~31128 &    SG &       5630 &       3.60 &      -1.87 &      -1.92 &          0 &         -- &      -0.15 &       0.11 &          4 &            &          0 &         -- &       0.04 &       0.23 &          5 \\ 
       HD~45282 &    RG &       5230 &       2.90 &      -1.59 &      -1.73 &          0 &         -- &      -0.24 &        0.10 &          4 &            &          0 &         -- &       0.12 &       0.18 &          5 \\ 
        HD~6268 &    RG &       4570 &       0.70 &      -2.82 &      -2.69 &          0 &         -- &      -0.31 &       0.09 &          4 &            &          0 &         -- &       0.01 &        0.20 &          7 \\ 
       HD~88609 &    RG &       4430 &       0.50 &      -3.29 &      -3.08 &          0 &         -- &      -0.37 &        0.10 &          3 &            &          0 &         -- &      -0.08 &        0.20 &          4 \\ 
       HD~94028 &    SG &       5730 &       3.70 &      -1.76 &      -1.81 &          0 &         -- &      -0.11 &        0.1 &          2 &            &          0 &         -- &       0.14 &       0.26 &          5 \\ 
 HE~0454$-$4758 &    RG &       5140 &       2.40 &      -3.38 &      -3.32 &          0 &         -- &       0.24 &       0.18 &          2 &            &          0 &         -- &       0.25 &       0.22 &          3 \\ 
 HE~0938$+$0114 &    SG &       6030 &       3.65 &      -3.09 &      -2.92 &          1 &    4379.23 &       0.93 &         -- &          0 &            &          1 &   3951.957 &       0.82 &         -- &          0 \\ 
 HE~1012$-$1540 &    RG &       5230 &       2.65 &      -4.17 &      -3.76 &          1 &    4379.23 &       1.42 &         -- &          0 &            &          1 &   3715.464 &       1.13 &         -- &          0 \\ 
 HE~1124$-$2335 &    RG &       4870 &       1.65 &      -3.36 &      -3.26 &          0 &         -- &      -0.21 &       0.18 &          1 &            &          0 &         -- &       0.08 &       0.21 &          4 \\ 
 HE~1320$-$1339 &    RG &       4690 &       1.20 &      -3.18 &      -2.93 &          0 &         -- &      -0.07 &        0.10 &          4 &            &          0 &         -- &       0.11 &       0.18 &          7 \\ 
 HE~1320$-$1339 &    RG &       4690 &       1.20 &      -3.18 &      -2.93 &          0 &         -- &      -0.09 &        0.10 &          4 &            &          0 &         -- &       0.04 &       0.19 &          3 \\ 
      HIP~99423 &    SG &       5520 &       3.70 &      -1.73 &      -1.42 &          0 &         -- &      -0.15 &        0.10 &          4 &            &          0 &         -- &       0.09 &       0.21 &          5 \\ 
\enddata      
\tablecomments{%
The final Vanadium abundances measurements for all 313 stars
and the corresponding uncertainties.
The model uncertainty is included in here.
}
\tablenotetext{a}{Flag for upper limit. ``1'' means only an upper limit is available.}
\end{deluxetable*}

